It's Time to Play Safe: Shield Synthesis for Timed Systems

Erroneous behaviour in safety critical real-time systems may inflict serious consequences. In this paper, we show how to synthesize timed shields from timed safety properties given as timed automata. A timed shield enforces the safety of a running system while interfering with the system as little as possible. We present timed post-shields and timed pre-shields. A timed pre-shield is placed before the system and provides a set of safe outputs. This set restricts the choices of the system. A timed post-shield is implemented after the system. It monitors the system and corrects the system's output only if necessary. We further extend the timed post-shield construction to provide a guarantee on the recovery phase, i.e., the time between a specification violation and the point at which full control can be handed back to the system. In our experimental results, we use timed post-shields to ensure the safety in a reinforcement learning setting for controlling a platoon of cars, during the learning and execution phase, and study the effect.

==> Shield Synthesis for Timed Systems/conclusion.tex <==
 We presented timed post-shields and timed pre-shields. 
 These are shields for real-time systems which can be attached either before or after a system, correcting the outputs received by the environment. 
 In addition, we discussed how timed shields can be used in reinforcement learning settings. 
 We presented a case study of a platoon of cars, and demonstrated the potential of a timed post-shield in RL. 
In the future, we would like to extend this work into several different directions.
First, we see great potential for shields
 in RL. In future work, we want to apply timed shields
on several challenging RL settings and investigate techniques for speeding up the learning performance in addition to providing safety.
Furthermore, we want to exploit techniques from model repair and model refinement
to deal with dynamic environments, and adapt the shields during runtime if needed.
In this work, we treat the system as adversary. In future work, we plan to study ways to model the spectrum between cooperative and adversarial systems to be shielded.

\iffalse
 While the shielding during the learning phase did not yield beneficial results, shielding during the execution phase avoided all crashes, while in the most complex setting, the unshielded system crashed in $98\%$ of the simulations.
Post shields are most permissive, and might thus offer a choice between multiple outputs in a given state. 
We leave it up for future work, to identify heuristics or apply machine learning, to identify which option is most beneficial.
\fi

==> Shield Synthesis for Timed Systems/definitions.tex <==
%In this section, we recall definitions in the field of real-time systems. We will address the definition of timed input/output automata, their usage as a  specification theory and timed game automata. 

Let us recall definitions of Timed (Input/Output) Automata.
%We will address the definition of timed input/output automata, their usage as a  specification theory and timed game automata. 
%
%We start by defining a framework for a set of real-valued variables $\clocks$, called \emph{clocks}.
Let $\clocks$ be a finite set of real-valued \emph{clocks}.
Let $\vals{\clocks}\mapsto\R$ be the valuations over $\clocks$ and let $\overset{\rightarrow}{0}$ be the valuation that assigns $0$ to each clock.
For the value of a single clock of a given valuation $\val\in\vals{\clocks}$, we write $\val(\uppClock{x})$ and $\val[\uppClock{x}]$ denotes the reset of the clock $\uppClock{x}$ in the valuation $\val$.
We extend the notion of reset to sets, i.e., for some $Y\subseteq \clocks$ let $\val[Y]$ be the valuation after resetting all values of clocks in $Y$ to zero
and otherwise retaining their value.
If $\delta\in \R$ is a positive delay, then we denote by $\val+\delta$ the valuation s.t. for all $\uppClock{x}\in X$, $(\val + \delta)(\uppClock{x})=\val(\uppClock{x})+\delta$.

Let $Y \subseteq \clocks $ and $Z \subseteq \clocks \cup \mathbb{Z} $. We denote the set of all simple constraints as $\Phi(Y, Z)=Y\times\{\uppProp{<,\leq,\geq, >}\}\times Z$.
The set of all  possible clock constraints is defined by $\constraints(\clocks)=2^{\Phi(\clocks, \clocks\cup\mathbb{Z})}$.
We denote the (conjunctive) subset of restricted clock constraints by $\cconstraints(X)\subseteq\constraints(X)$ with $\cconstraints(X)= 2^{\Phi(\clocks,\mathbb{Z})}$.


%Let $\psi\in\constraints(\clocks)$ be a set of constraints over the clocks $\clocks$ and let $\val\in\vals{\clocks}$ be a given valuation. We write $\val\models\psi$,  if for all $\phi\in\psi$ we have that
%$\val$ satisfies $\phi$.
%For the set of values satisfying a given constraint $\psi$, we write $\semof{\psi}=\{\psi\in\vals{\clocks} \mid \val\models\psi\}$. As a shorthand, we write $\true$ if $\psi=\emptyset$ and $\false$, if for all $\val\in\vals{\clocks}$ we have $\val\not\models\psi$.
%Without loss of generality, we assume that all constraints are minimal, implying that if $\psi\neq\emptyset$, then for any $\phi\in\psi$ we have $\semof{\psi}\subset\semof{\psi\setminus\phi}$.

%We denote by $\overline{\psi}\subseteq \cconstraints(\clocks)$ the complement of a clock-constraint $\psi\in\cconstraints(\clocks)$ which is defined as a set of (conjunctive) clock constraints.
%Similarly, we let conjunctions of sets of clock-constraints be defined using standard notation: If $\psi,\psi\subseteq \cconstraints(\clocks)$, then $\semof{\psi}\cap\semof{\psi'}\subseteq\cconstraints(\clocks)$. If $\nu\models\semof{\psi}\cap\semof{\psi'}$, then $\nu\models\psi$ and $\nu\models\psi'$.

% We also define the ``last boundary'' operator $\lastbound:\cconstraints(\clocks)\rightarrow2^{\cconstraints(\clocks)}$ of a constraint $\psi\in\cconstraints(\clocks)$ recursively as follows.
% $$
% \lastbound(\psi)=\begin{cases}
% \emptyset  &\text{ if }\psi=\true,\\
% \{\{(x,>,y),(x,<,y)\}\}\cup\lastbound(\psi\setminus\{(x,<, y)\})&\\&\text{ if }(x,<, y)\in\psi,\\
% \{\{(x,\geq,y),(x,\leq,y)\}\}\cup\lastbound(\psi\setminus\{(x,\leq, y)\})&\\&\text{ if }(x,\leq, y)\in\psi, \text{and}\\
% \lastbound(\psi\setminus\{\phi\}) &\text{ for }\phi\in\psi\text{ matching neither.}
% \end{cases}
% $$
%The intuition behind the last boundary operator is to reduce a constraint to the last point in time, where the constraint $\psi$ is still satisfied.
%An example would be $\lastbound(\{(x,\leq, 2),(y,\leq 3,)\})=\{\{(x,\leq, 2),(x,\geq, 2)\},\{(y,\leq 3,),(y,\geq 3,)\}\}$ where a satisfying valuation either has $x=2$ or $y=3$.


\begin{definition}[Timed Input/Output Automaton (TIOA)~\cite{alur1994theory, david2010timed}]
A Timed Input/Output Automaton (TIOA) is a tuple $\A=(\locs,\loc_0,\taactions{}^?,\taactions{}^!,\clocks,\edges,\invars)$ where
	$\locs$ is a finite set of locations,
	$\loc_0$ is the initial location,
	$\taactions{}=\taactions{}^?\cup\taactions{}^!$ is a finite
   set of actions partitioned into inputs ($\taactions{}^?$) and outputs ($\taactions{}^?$),
	 $\clocks$ is a set of clocks,
	 $\edges\subseteq \locs\times\cconstraints(\clocks)\times(\taactions{}^!\cup\taactions{}^?)\times2^{\clocks} \times \locs$ 
	 is a set of edges, and % consisting of a source-location, a clock guard, an action, a set of clocks to reset, and a target location.
	$\invars:\locs\rightarrow\cconstraints(\clocks)$ is a function assigning invariants to locations.
\end{definition}
%
States of a TIOA are given as a pair $(\loc,\val)\in \locs\times\mathbb{R}_{\geq_0}^{\clocks}$ consisting of a discrete location and a real-valued assignment to the clocks.
From a given state $(\loc,\val)\in \locs\times\mathbb{R}_{\geq_0}^{\clocks{}}$ where $\val\models\invars(\loc)$, we have two kinds of transitions; (1) \emph{discrete transitions}: $(\loc,\val)\trans{\alpha}(\loc',\val')$ if there exists $(\loc,\psi,\alpha,Y,\loc')\in \edges$ s.t. $\val\models \psi$, $\val'=\val[Y]$ and $\val'\models\invars(\loc')$, and
	(2) \emph{delay transitions} for some $\delta\in \R$ where $(\loc,\val)\trans{\delta}(\loc,\val')$ if $\val'=\val+\delta$ and $\val'\models\invars(\loc)$.
%
We define the semantics of a TIOA as a TLTS.
%
\begin{definition}[Timed Labeled Transitions System (TLTS)~\cite{alur1994theory, david2010timed}]
A TLTS is a tuple $\llbracket \A \rrbracket=(\Q,q_0,\rightarrow)$ s.t. $\Q=\locs\times\mathbb{R}_{\geq_0}^{\clocks{}}$, $q_0=(\loc_0,\overset{\rightarrow}{0})$,
and $\rightarrow: Q \times \taactions^!{}\cup\taactions^?{}\cup\R \times Q $ is a transition relation defined  as above.
\end{definition}
%
A {\em trace} $\sigma$ of an TIOA is a finite sequence of alternating delay and discrete transitions of the form
$(l_{0}, v_{0}) \xrightarrow{\delta_1} (l_{0}, v_{0} + \delta_{1}) \xrightarrow{\tau_{1}} (l_{1}, v_{1}) \xrightarrow{\delta_{2}} \cdots
\xrightarrow{\delta_{n}} (l_{n-1}, v_{n-1} + \delta_{n}) \xrightarrow{\tau_{n}} (l_{n}, v_{n})$,
where $v_{0} = \overset{\rightarrow}{0}$ and $\tau_{i} = (l_{i-1}, \alpha_{i}, g_{i},  Y, l_{i}) \in \edges$. By agreement we let $\trans{\ast}$ denote the transitive closure of the transition-function.

%For a trace $\sigma$ we let $out(\sigma) = \delta_0 \cdot \alpha_0 \cdot \dots \cdot  \delta_n \cdot \alpha_n $ denote the timed sequence of outputs of a trace where $n$ is the number of outputs in $\sigma$. Furthermore, for each $k<n$ we have that $\alpha_k$ is the k-th output in $\sigma$, and $\delta_k$ is the sum of the delays in $\sigma$ since the (k-1)-th output in $\sigma$. We denote by $out(\A)$ the set of timed sequences for all traces of $\A$. We denote by $out_t(\sigma)$ and $out_t(\A)$ the timed sequence of outputs and set of timed sequences of outputs, starting from time $t$. 

The state space of TIOA can be represented via \emph{zones}~\cite{alur1994theory}, symbolic sets of states containing the max. set of clock valuations satisfying given constraints. 

In this paper, we only consider deterministic and input enabled TIOA.
$\A$ is \textit{deterministic}, if $\llbracket \A \rrbracket$ satisfies that $\forall \alpha \in \taactions{}, \forall (\loc,\val) \in \Q . (\loc,\val)\trans{\alpha}(\loc',\val') \wedge (\loc,\val)\trans{\alpha}(\loc'',\val'') \implies \loc' = \loc'' \wedge \val' = \val''$. Thus, in every state,  transitions of a given label will lead to a unique state. 
$\A$ is \textit{input-enabled}, if $\llbracket \A \rrbracket$ satisfies that $\forall \alpha \in \taactions{}^?, \forall (\loc,\val) \in \Q . (\loc,\val)\trans{\alpha}(\loc',\val')$. 
Thus, every state can receive any input.  For simplicity, we assume implicit input-enabledness in our figures.

TIOA can be used as \emph{specifications}. %for systems. Generally, 
Specifications are not necessarily exact on timing behaviour (e.g., on the output of a label) but allow for ranges of timing. 
An \emph{implementation} satisfies a specification as long as any behavior is included in that of the specification.

\begin{figure}[tb]
	
	\minipage{0.49\textwidth}
	\centering
	\includegraphics[width=0.7\linewidth]{images/Spec-eps-converted-to.pdf}\\
	(a)
	\endminipage\hfill
	\minipage{0.49\textwidth}
	\centering
	\includegraphics[width=0.7\linewidth]{images/ref-eps-converted-to.pdf}\\
	(b)
	\endminipage\hfill
	\caption{Specification $\spec_1$ (a) of a light switch; specification $\spec_2$ refines it (b).}
	\label{fig:example_kim}
	\vspace{-10pt}
\end{figure}

\textbf{Example.} \emph{Fig.~\ref{fig:example_kim}(a) shows a specification  $\spec_1$ of a light switch: whenever the light is switched \uppLoc{ON},  this setting has to be kept for $1$ to $5$ time units. Whenever the light is switched \uppLoc{OFF}, the light switch has to blink at least once every $3$ time units. The timing is tracked via the clock $\uppClock{x}$.}
%


We say that a TIOA $\A_\mathcal{I}$ \emph{refines} a TIOA $\A_\mathcal{S}$ if the corresponding TLTS $\llbracket \A_\mathcal{I} \rrbracket$ refines the TLTS $\llbracket\A_\mathcal{S} \rrbracket$, let us formally defined this relationship.

\begin{definition}[Refinement\cite{david2010timed}] \label{def:ref}
A TLTS $\mathcal{I}=(\Q_\mathcal{I},q_0^\mathcal{I},\rightarrow_\mathcal{I}) $ refines a TLTS $\mathcal{S}=(\Q_\mathcal{S},q_0^\mathcal{S},\rightarrow_\mathcal{S})$, written $\mathcal{I} \leq \mathcal{S}$, iff there exists a binary relation $R\subseteq \Q_\mathcal{I} \times \Q_\mathcal{S}$ containing $(q_0^\mathcal{I},q_0^\mathcal{S})$ such that for each pair of states $(q_\mathcal{I},q_\mathcal{S}) \in R$ we have:
\begin{enumerate}
%\item if $q_\mathcal{S}  \xrightarrow{i?}_\mathcal{S} q'_\mathcal{S}$ for some $q'_\mathcal{S} \in \Q_\mathcal{S}$ then $q_\mathcal{I}  \xrightarrow{i?}_\mathcal{I} q'_\mathcal{I}$ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$  for some $q'_\mathcal{I} \in \Q_\mathcal{I}$,
\item if $\exists q'_\mathcal{S} \in \Q_\mathcal{S}. ~q_\mathcal{S}  \xrightarrow{i?}_\mathcal{S} q'_\mathcal{S}$
 then $\exists q'_\mathcal{I} \in \Q_\mathcal{I}. ~
  q_\mathcal{I}  \xrightarrow{i?}_\mathcal{I} q'_\mathcal{I}$ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$
\item if $\exists q'_\mathcal{I} \in \Q_\mathcal{I}. q_\mathcal{I}  \xrightarrow{o!}_\mathcal{I} q'_\mathcal{I}$ then $\exists q'_\mathcal{S} \in \Q_\mathcal{S}. q_\mathcal{S}  \xrightarrow{o!}_\mathcal{S} q'_\mathcal{S} $ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$ and 	
\item if $\exists \delta \in \mathbb{R}_{\geq 0}. q_\mathcal{I}  \xrightarrow{\delta}_\mathcal{I} q'_\mathcal{I}$ then $q_\mathcal{S}  \xrightarrow{\delta}_\mathcal{S} q'_\mathcal{S}$ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$.

\end{enumerate}
\end{definition}
%

\textbf{Example.} \emph{Fig.~\ref{fig:example_kim}(b) shows a specification  $\spec_2$ 
that refines the specification $\spec_1$ of Fig~\ref{fig:example_kim}(a) by restricting the timings of some of the signals.}
%

Given a specification \spec and a system \sys, a \textbf{monitor} \mspec observes
\sys w.r.t \spec (i.e., all transitions in \mspec are inputs) and enters an
error-state \uppLoc{ERR} whenever non-conformance between \sys and \spec is observed, that is, whenever
an output of \sys is observed that is not allowed by \spec.
\begin{figure}[tb]	
	\centering
	\includegraphics[width=0.59\linewidth]{images/mSpec-eps-converted-to.pdf}	
	\caption{A monitor \mspec of the light switch specification $\spec_1$ of Fig.~\ref{fig:example_kim}(a).}
	\label{fig:mon}
	\vspace{-10pt}
\end{figure}

\textbf{Example. }\emph{Fig.~\ref{fig:mon} depicts a monitor for $\spec_1$ of Fig.~\ref{fig:example_kim}(a).% Note, that due to the implicit input-enabledness there is no transition for \uppIn{on} in the \uppLoc{ON} location in either \spec or \mspec.
}

We use \emph{Networks of Timed Automata} to enable parallel composition of TIOA. 
%
\begin{definition}[Networks of Timed Automata (NTA)~\cite{alur1994theory}]
%
Let $\Sigma$ be a set of actions and let $\Sigma_1,\dots,\Sigma_n$ be a partitioning of $\Sigma$. 
Let $\A_1,\A_2,\dots,\A_n$ be TIOAs, where $\llbracket \A_i \rrbracket = (\Q^i,q_0^i,\rightarrow^i)$
and $\A_i$ has $\Sigma_i$ as its output and $\Sigma$ as its input alphabet.
A network of TIOA $\A_1\|\A_2\| \dots \| \A_n$ is defined via the 
TLTS $(\Q^1\times\dots\times\Q^n,(q_0^1,... , q_0^n),\rightarrow)$ with:
%
$$\frac{[s_i \xrightarrow{\delta}_i s'_i]_{i=1 \dots n}}{(s_1, \dots, s_n) \xrightarrow{\delta}  (s'_1, \dots, s'_n)}~~\text{with } \delta \in \R \text{, and}$$
$$\frac{[s_j \xrightarrow{\alpha!}_j s'_j] [s_i \xrightarrow{\alpha?}_i s'_i]_{i \neq j}}{(s_1, \dots, s_n) \xrightarrow{\alpha!}  (s'_1, \dots, s'_n)}~~\text{with }{\alpha \in \Sigma_j}.$$ 
\end{definition}
%
For deterministic specifications, the following important theorem, given in the syntax of \uppaal queries~\cite{behrmann2004tutorial}, holds, stating that a system refines a specification iff the parallel product of the system and the specification monitor cannot reach the error-state.
\begin{theorem}
	$\forall~ \sys.~ \sys \leq \spec~~$ iff $~~(\sys ~|~ \mspec) \models A \Box~ \neg
	\mspec.\uppLoc{ERR} $
\end{theorem}


\begin{definition}[Timed Game Automaton (TGA)~\cite{maler1995synthesis}]
 A Timed Game Automaton (TGA) is a TIOA in which the set of output actions $\taactions^{!}$ is partitioned into controllable actions ($\taactions_C$) and uncontrollable actions ($\taactions_U$).
\end{definition}
The definition of NTA trivially extends to Networks of TGA (NTGA).

%Ask Flo if this is needed!????
%For NTGA, different synchronization semantics arise when sender and receiver actions are under the control of different players.
%In this paper, we assume the semantics that the player of the sending transitions of a synchronization is forced upon receiving transitions and therefore only partition the sending actions into controllable and uncontrollable, thus avoiding ambiguous interpretations.
%
%\begin{definition}[Memoryless Strategy]
Given a TGA $\mathcal{G}=(\langle\locs,\loc_0,\taactions{},\clocks,\edges,\invars,\rangle,$ $\taactions_U,\taactions_C)$, a \emph{memoryless strategy} $\omega:\locs{}\times\mathbb{R}_{\geq_0}^{\clocks{}}\rightharpoonup 2^{\{\lambda\}\cup\taactions{}_C}$ is a  function over the states of $\mathcal{G}$ to the set of controllable actions or a special nothing-symbol $\tau$.
%\end{definition}
%ask Flo: Tau or Lambda????

\begin{definition}[Strategy Composition]
Given a TGA $\mathcal{G}=(\langle\locs,\loc_0,\taactions{},\clocks,\edges,\invars,\rangle,$ $\taactions_U,\taactions_C)$ and a memoryless strategy $\omega$, the composition $\mathcal{G}\|\omega$ provides a restriction of the transition-system of $\mathcal{G}$;
\begin{itemize}
	\item if $(\loc,\val)\trans{\alpha}(\loc',\val')$ then either we have $\alpha\in\Sigma^?$ or we have $\alpha\in\Sigma^!$ and $\alpha\not\in\taactions_C$ or $\alpha\in\omega(\loc,\val)$, and
	
		\item if $(\loc,\val)\trans{\delta}(\loc',\val')$  for $\delta\in\R$ then $\forall \delta'<\delta$ it holds that $\lambda\in\omega(\loc,\val+\delta')$.
	
	
\end{itemize}
\end{definition}

Let $\varphi\subseteq\locs$ be a set of losing locations for a TGA $\mathcal{G}$. The \textit{safety control problem} consists in finding a strategy $\omega$, s.t. $\mathcal{G}\|\omega$ constantly avoids $\varphi$. A trace $\sigma= (l_{0}, v_{0}) \xrightarrow{\delta_1} (l_{0}, v_{0} + \delta_{1}) \cdots
\xrightarrow{\delta_{n}} (l_{n-1}, v_{n-1} + \delta_{n}) \xrightarrow{\tau_{n}} (l_{n}, v_{n})$ is \textit{winning} if  $\forall k \leq n : l_k \notin \varphi$. A strategy $\omega$  is winning, if all traces of $\mathcal{G}\|\omega$ are winning.

We denote by $\wrm\subseteq\locs\times\mathbb{R}_{\geq_0}$ the \emph{winning region}, i.e., the set of all states $s$ such that there exists a winning strategy from $s$. We denote by \emph{correct} (\emph{wrong}) outputs for a state $s$ the outputs that lead to an $s' \in \wrm$  ($s' \not\in \wrm$, respectively). We denote by $\swr$ the set of states  in $\wrm$, such that any delay would leave $\wrm$.

%The \uppaal tool suite provides support for TIOA and TGA with the tools \uppaalecdar~\cite{david2010ecdar} and \uppaaltiga~\cite{CassezDFLL05}, respectively. The tools use zones as an efficient representation of the state-space of timed automata.






%, then we can define a maximal set of winning states $\mathcal{W}$ as the maximal fix-point with;
%\begin{itemize}
%	 \item $\mathcal{W}_0=\{(\loc,\nu)\mid\loc\in\varphi\text{ and }\nu\in\mathbb{R}_{\geq_0}^{\clocks{}}\}$, and
%	 \item $\mathcal{W}_n=\{(\loc,\nu)\mid\text{ for all }(\loc',\nu')\text{ where }(\loc,\nu)\underset{\mathcal{G}\|\omega}{\rightarrow}(\loc',\nu')\text{ we have }(\loc',\nu')\in\mathcal{W}_{n-1}\}$.
% \end{itemize}
% \todo[inline]{Definition of cooperative might not be needed, and same for the text below, other than the winning strategy}


%A strategy is winning if $(\loc_0,\overset{\rightarrow}{0})\in\mathcal{W}$.

%\todo[inline]{Preliminaries about UPPAAL, TIGA, Regions, Zones}




\iffalse
\textbf{Before Tina touched it!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!}
\begin{definition}[Timed Input/Output Automaton~\cite{alur1994theory, david2010timed}]
A Timed Input/Output Automaton (TIOA) is a tuple $\A=(\locs,\loc_0,\taactions{}^?,\taactions{}^!,\clocks,\edges,\invars)$ where
\begin{itemize}
	\item $\locs$ is a finite set of locations,
	\item $\loc_0$ is the initial location,
	\item ($\taactions{}^?$) and ($\taactions{}^!$) are sets of input and output actions postfixed by $!$ and $?$, respectively, which together form the set of actions $\taactions{}=\taactions{}^?\cup\taactions{}^!$,
	\item $\clocks$ is a set of clocks,
	\item $\edges\subseteq \locs\times\cconstraints(\clocks)\times(\taactions{}^!\cup\taactions{}^?)\times2^{\clocks} \times \locs$ is a set of edges consisting of a source-location, a clock guard, an action, a set of clocks to reset, and a target location.
	\item $\invars:\locs\rightarrow\cconstraints(\clocks)$ is a function assigning invariants to locations.
\end{itemize}
\end{definition}



States of a TIOA are given as a pair $(\loc,\val)\in \locs\times\mathbb{R}_{\geq_0}^{\clocks}$ consisting of a discrete location and a real-valued assignment to the clocks.
From a given state $(\loc,\val)\in \locs\times\mathbb{R}_{\geq_0}^{\clocks{}}$ where $\val\models\invars(\loc)$ we have two kinds of transitions;
\begin{itemize}
	\item discrete transitions, $(\loc,\val)\trans{\alpha}(\loc',\val')$ if there exists $(\loc,\psi,\alpha,Y,\loc')\in \edges$ s.t. $\val\models \psi$, $\val'=\val[Y]$ and $\val'\models\invars(\loc')$, and
	\item delay transitions for some $\delta\in \R$ where $(\loc,\val)\trans{\delta}(\loc,\val')$ if $\val'=\val+\delta$ and $\val'\models\invars(\loc)$.
\end{itemize}

We can therefore define the semantics of a TIOA $\mathcal{A}$ as a Timed Labeled Transitions System (TLTS) $\llbracket \A \rrbracket=(\Q,q_0,\rightarrow)$ s.t. $\Q=\locs\times\mathbb{R}_{\geq_0}^{\clocks{}}$, $q_0=(\loc_0,\overset{\rightarrow}{0})$ with the transition relation defined as above and the set of labels given by $\taactions^!{}\cup\taactions^?{}\cup\R$.

A {\em trace} $\sigma$ of an TIOA $\A$ is a finite sequence of alternating timed and discrete transitions of the form
$(l_{0}, v_{0}) \xrightarrow{\delta_1} (l_{0}, v_{0} + \delta_{1}) \xrightarrow{\tau_{1}} (l_{1}, v_{1}) \xrightarrow{\delta_{2}} \cdots
\xrightarrow{\delta_{n}} (l_{n-1}, v_{n-1} + \delta_{n}) \xrightarrow{\tau_{n}} (l_{n}, v_{n})$,
where $v_{0} = \overset{\rightarrow}{0}$ and $\tau_{i} = (l_{i-1}, \alpha_{i}, g_{i},  Y, l_{i}) \in \edges$.

By agreement we let $\trans{\ast}$ denote the transitive closure of the transition-function.

A TIOA $\A$ is \textit{deterministic}, if $\llbracket \A \rrbracket$ satisfies that $\forall (\loc,\val) \in \Q . (\loc,\val)\trans{\alpha}(\loc',\val') \wedge (\loc,\val)\trans{\alpha}(\loc'',\val'') \implies \loc' = \loc'' \wedge \val' = \val''$. Thus, in every state,  transitions of a specific label will lead to the same state.


A TIOA $\A$ is \textit{input-enabled}, if $\llbracket \A \rrbracket$ satisfies that $\forall \alpha \in \taactions{}^?, \forall (\loc,\val) \in \Q . (\loc,\val)\trans{\alpha}(\loc',\val')$. 
Thus, every state can receive any input.

In this paper we only consider deterministic and input enabled TIOA.

Timed input output automata can be uses as specifications for systems. Generally, specifications are not strict on timing behavior and allow for ranges of timing, instead requiring that a transition has to be taken at an exact point of time. This allows for implementations to choose any concrete behavior, as long as their behavior is included in the specification. 

Figure~\ref{fig:example_kim}(a) shows an example of a specification automaton of a light switch: whenever the light is switched \uppLoc{ON},  this setting has to be kept for $1$ to $5$ time units, and whenever the light is switched \uppLoc{OFF}, the light switch has to blink at least once every $3$ time units. The timing is tracked via the clock $\uppClock{x}$.

\begin{figure}[tb]
	
	\minipage{0.49\textwidth}
	\centering
	\includegraphics[width=0.7\linewidth]{images/Spec-eps-converted-to.pdf}\\
	(a)
	\endminipage\hfill
	\minipage{0.49\textwidth}
	\centering
	\includegraphics[width=0.7\linewidth]{images/ref.eps}\\
	(b)
	\endminipage\hfill
%	\\
%	\minipage{0.49\textwidth}
%	\centering
%	\includegraphics[width=0.7\linewidth]{images/Specp}\\
%	(c)
%	\endminipage\hfill
%	\minipage{0.49\textwidth}
%	\centering
%	\includegraphics[width=0.99\linewidth]{images/mSpecp}\\
%	(d)
%	\endminipage\hfill
	
	\caption{Specification (a) of a light switch and a specification refining it (b).}
	\label{fig:example_kim}
\end{figure}



%We distinguish between implementations and specifications~\cite{ulrik} by adding conditions on the timed automata. This is done by assuming that the former have %fixed timing behaviour and they can always advance either by producing an output or delaying. In contrast, specifications are more general and allow ranges of %timed behavior.

Furthermore, we need a \textit{refinement} relation between specifications~\cite{david2010timed}.
%A TA $A_1$ refines a TA $A_2$ if and only if it is possible to replace $A_2$ with $A_1$ in every environment and obtain an equivalent system.
The formal definition of refinement for specifications is based on the underlying labeled transition systems.

\begin{definition}[Refinement]

\label{def:ref}
A TLTS $\mathcal{I}=(\Q_\mathcal{I},q_0^\mathcal{I},\rightarrow_\mathcal{I}) $ refines a TLTS $\mathcal{S}=(\Q_\mathcal{S},q_0^\mathcal{S},\rightarrow_\mathcal{S})$, written $\mathcal{I} \leq \mathcal{S}$, iff there exists a binary relation $R\subseteq \Q_\mathcal{I} \times \Q_\mathcal{S}$ containing $(q_0^\mathcal{I},q_0^\mathcal{S})$ such that for each pair of states $(q_\mathcal{I},q_\mathcal{S}) \in R$ we have:
\begin{enumerate}

\item whenever $q_\mathcal{S}  \xrightarrow{i?} q'_\mathcal{S} \in \rightarrow_\mathcal{S}$ for some $q'_\mathcal{S} \in \Q_\mathcal{S}$ then $q_\mathcal{I}  \xrightarrow{i?} q'_\mathcal{I} \in \rightarrow_\mathcal{I}$ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$  for some $q'_\mathcal{I} \in \Q_\mathcal{I}$
\item whenever $q_\mathcal{I}  \xrightarrow{o!} q'_\mathcal{I} \in \rightarrow_\mathcal{I}$ for some $q'_\mathcal{I} \in \Q_\mathcal{I}$ then $q_\mathcal{S}  \xrightarrow{o!} q'_\mathcal{S} \in \rightarrow_\mathcal{S}$ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$  for some $q'_\mathcal{S} \in \Q_\mathcal{S}$ 	
\item whenever $q_\mathcal{I}  \xrightarrow{\delta} q'_\mathcal{I} \in \rightarrow_\mathcal{I}$ for some $\delta \in \mathbb{R}_{\geq 0}$ then $q_\mathcal{S}  \xrightarrow{d} q'_\mathcal{S} \in \rightarrow_\mathcal{S}$ and $(q'_\mathcal{I},q'_\mathcal{S}) \in R$  for some $q'_\mathcal{S} \in \Q_\mathcal{S}$
\end{enumerate}
Consequently, a specification $\A_\mathcal{I}$ refines a specification $\A_\mathcal{S}$ if the corresponding LTS$\llbracket \A_\mathcal{I} \rrbracket$ refines the corresponding LTS $\llbracket\ A_\mathcal{S} \rrbracket$.
\end{definition}

Figure~\ref{fig:example_kim}(b) shows a specification of the light switch refining the specification shown in Figure~\ref{fig:example_kim}(a), by restricting the timings of some of the signals.

\begin{figure}[tb]	
	\centering
	\includegraphics[width=0.59\linewidth]{images/mSpec.eps}	
	\caption{A monitor of the light switch specification.}
	\label{fig:mon}
\end{figure}



Given any specification \spec, we may construct a \textbf{monitor} \mspec (as seen in Figure~\ref{fig:mon}), which only observes
the system \sys (i.e., all transitions in \mspec are inputs) and enters an
error-state \uppLoc{ERR} whenever non-conformance is observed, that is, whenever
an output is observed that is not allowed in the original \spec in the given situation. Note that, in order to make the figures simpler, we assume implicit input-enabledness, and every input not defined in \spec is ignored, which is taken over for \mspec. Thus, there is no transition for \uppIn{on} in the \uppLoc{ON} location in either \spec or \mspec.



% The intuition behind the quotient operator is as follows: given a global specification T of a composite system as well as the specification of an already realized component S, the quotient will return the most liberal specification X for the missing component, i.e. X is the largest
% specification such that S in parallel with X refines T.

% Formally, quotienting for two timed automata $A_T = (\locs[T],\loc_0^T,\taactions{}_T^?,\taactions{}_T^!,\clocks_T,\edges_T,\invars[T],\comitted_T)$ and $A_S = (\locs[S],\loc_0^S,\taactions{}_S^?,\taactions{}_S^!,\clocks_S,\edges_S,\invars[S],\comitted_S)$ is defined in the following way. The quotient, which is denoted $A_T \setminus A_S$
% is the TA given by: $\locs = \locs[T] \times \locs[S] \cup \{l_u,l_{\emptyset}\}, \loc_0 = (\loc_0^T, \loc_0^S), \clocks = \clocks_T \cup \clocks_T \cup \{x_{new}\}, \invars = Inv(l_u) = \textrm{true and} Inv(l_{\emptyset}) = {x_{new} \leq 0}$. The two new states $l_u$ and $l_{\emptyset}$ are respectively universal and inconsistent. The set of actions $\taactions{} = \taactions{}^? \cup \taactions{}^!$ is given by $\taactions{}^? = \taactions{}_T^? \cup \taactions{}_S^! \cup \{i_{new}\}$ and $\taactions{}^! = \taactions{}_T^! \\ \taactions{}_S^!$.
% The set of edges $\edges$ is defined by the following rules:

% \begin{itemize}
% \item For each $\loc_T \in \locs[T] , loc_S \in \locs[S]$ and $a \in \taactions{}$ this gives
% $((\loc_T , \loc_S), \neg \invars[S](\loc_S), \alpha, \{x_{new}\}, l_u) \in \edges$.
% \item For each $\loc_T \in \locs[T], \loc_S \in \locs[S]$ this gives
% $((\loc_T , \loc_S), \neg \invars[T](\loc_T ) \vee \invars[S](\loc_S), i_{new}, \{x_{new}\}, l_{\emptyset}) \in \edges$.
% \item If $(\loc_T ,\psi_T,\alpha_T, Y_T, \loc'_T) \in \edges_T$ and $(\loc_S, \psi_S, \alpha_S, Y_S, \loc'_S)  \in \edges_S$ this gives $((\loc_T , \loc_S), \psi_T \wedge \psi_S, \alpha, Y_T \cup Y_S,(\loc'_T , \loc'_S)) \in \edges$.

% \item For each $(\loc_S, \psi_S, \alpha, Y_S, \loc'_S)  \in \edges_S$ with $\alpha \in \taactions{}_S^!$ this
% gives rise to $(((\loc_T , \loc_S), \psi_S \wedge \neg G_T, \alpha, \{\},\loc_{\emptyset})$ where $G_T = \bigvee \{\psi_T | (\loc_T , \alpha, \psi_T , Y_T , \loc'_T)\}$

% \item For each $(\loc_T ,\psi_T,\alpha, Y_T, \loc'_T) \in \edges_T$ and $\alpha \notin \taactions{}_S$ this gives  $((\loc_T , \loc_S), \psi_T, \alpha, Y_T, (\loc'_T , \loc_S)) \in \edges$

% \item For each $(\loc_T ,\psi_T,\alpha, Y_T, \loc'_T) \in \edges_T$ and $\alpha \in \taactions{}_S^!$ this gives  $((\loc_T , \loc_S), \neg G_S, \alpha, \{\}, \loc_u) \in \edges$ where  $G_S = \bigvee \{\psi_S | (\loc_S , \alpha, \psi_S , Y_S , \loc'_S)\}$


% \item For each $\alpha \in \taactions{}^?$ this gives rise to $(\loc_{\emptyset}, x_{new} == 0, \alpha, \{\}, \loc_{\emptyset})$

% \item For each $\alpha \in \taactions{}$ this gives rise to $(\loc_u, \alpha, true, \{\}, l_u)$

% \end{itemize}






To enable parallel composition of TIOA, \emph{Networks of Timed Automata} (NTAs) have been introduced.
%In this paper, we will use  so-called \emph{broadcast} semantics of synchronization exclusively, and thereby breaking subtly from conventional NTA semantics.

\begin{definition}[Composition of Timed Automata~\cite{alur1994theory}]

Let $\Sigma$ be a set of actions and let $\Sigma_1,\dots,\Sigma_n$ be a partitioning of $\Sigma$. Now we may compose the network of TIOA $\A_1,\dots,\A_n$, where $A_i$ has $\Sigma_i$ as output and $\Sigma$ as input.

Let $\llbracket \A_i \rrbracket = (\Q^i,q_0^i,\rightarrow^i)$, then $\llbracket \A_1 | ... | \A_n \rrbracket$ is the TLTS $(\bigtimes_i \Q^i,(q_0^1,... , q_0^n),\rightarrow)$ where

\minipage{0.39\textwidth}
	\centering
	\infer{(s_1, \dots, s_n) \xrightarrow{\delta}  (s'_1, \dots, s'_n)}{[s_i \xrightarrow{\delta}_i s'_i]_{i=1 \dots n}}\endminipage  ~~
\minipage{0.09\textwidth}${\delta \in \R}$
\endminipage ~~~~~~
\minipage{0.39\textwidth}
	\centering
\infer{(s_1, \dots, s_n) \xrightarrow{\alpha!}  (s'_1, \dots, s'_n)}{[s_j \xrightarrow{\alpha!}_j s'_j] [s_i \xrightarrow{\alpha?}_i s'_i]_{i \neq j}}
\endminipage  ~~
\minipage{0.09\textwidth}${\alpha \in \Sigma_j}$
\endminipage




\end{definition}



 For deterministic specifications, the following important theorem holds:
\begin{theorem}
	$\forall~ \sys~ \sys \leq \spec$ iff $(\sys ~|~ \mspec) \models A \box \neg
	\mspec.\uppLoc{ERR} $
\end{theorem}
Thus, \sys refines \spec if and only if the parallel product of \sys and \mspec can never reach the error-state.











% \begin{definition}[Network of Timed Automata~\cite{alur1994theory}]
% Let $\A_1,\A_2,\dots,\A_n$ be TA where $\A_i =
% (\locs[i],\initloc[i], \clocks_{i},\taactions{}_i,\edges_{i},
% \invars[i],\comitted_i)$.
 % We let $\states(\A_i) = \locs[i]\times
% \vals{\clocks_i}$; then we define the states of the network
% $\A_1\|\A_2\| \dots \| \A_n$ to be a tuple of states $(s_1,s_2,\dots,s_n)$ where if $(\ell_i,\nu_i)=s_i$.
% A network may transit from
% $(s_1,s_2,\dots,s_n)$ by
% \begin{itemize}
% \item a timed transition $(s_1,s_2,\dots s_n)\xrightarrow{d}
  % (s_1',\dots,s_n')$ if for all $i$, $(\ell_i, \val_i) \xrightarrow{d}(\ell_i, \val'_i)$ where
  % $(\ell_i,\val_i)=s_1$, $(\ell'_i,\val'_i)=s_2$, and
% \item a discrete transition $((\ell_1,\val_1),\dots, (\ell_n,\val_n))\xrightarrow[i]{\oaction{a}}
  % ((\ell'_1,\val'_1),\dots,(\ell'_n,\val'_n))$ if
  % \begin{enumerate}
        % \item $(\ell_i,\val_i)\xrightarrow{a!}(\ell'_i,\val'_i)$, and
        % \item for $j\in \{1,\dots,n\}\setminus\{i\}$ we have
        % $$(\ell_j,\val_j)\xrightarrow{a?}(\ell'_j,\val'_j)$$
        % and either $\comitted_i(\ell_i)=\true$ or for all $j\in \{1,\dots,n\}\setminus\{i\}$ we have $\comitted_j(\ell_j)=\false$.
   % \end{enumerate}
% \end{itemize}
% \end{definition}

% For a state $q=(s_1,\dots,s_n)$ of an NTA $ \N = \A_1\| \dots \| \A_n$, we let the function $\stateof_{\N}(i, q)=s_i$ yield us the state of the $i$'th TA in the product state $q$ for some $1\leq i \leq n$.
% Notice that the use of broadcast transitions makes all TAs in the NTA input-enabled, i.e. that they accept any input action even if an edge is not defined, meaning that an automaton with an undefined input action will not change state if another automaton outputs said action.
% By agreement, we let $(\N)_\Sigma$ denote the NTA $\N$ in which only delays and labels of $\Sigma$ are observable.

%We denote by $out(l)$ the outputs that can be produced in a given location, and by $out(\sigma)$ the outputs that can be produced after a given trace.

\begin{definition}[Timed Game Automaton~\cite{maler1995synthesis}]
 A Timed Game Automaton (TGA) is a TIOA in which the set of output actions $\taactions^{!}$ is partitioned into controllable actions ($\taactions_C$) and uncontrollable actions ($\taactions_U$).
\end{definition}
The definition of NTA trivially extends to Networks of TGA (NTGA).
In the normal semantic framework of NTGA, different synchronization semantics arise when the sender and receiver action are under the control of different players.
In this paper we assume the semantics that the player of the sending transitions of a synchronization is forced upon receiving transitions and therefore only partition the sending actions into controllable and uncontrollable, thus avoiding ambiguous interpretations.

\begin{definition}[Memoryless Strategy]
Given a TGA $\mathcal{G}=(\langle\locs,\loc_0,\taactions{},\clocks,\edges,\invars,\rangle,$ $\taactions_U,\taactions_C)$, a (memoryless) strategy $\omega:\locs{}\times\mathbb{R}_{\geq_0}^{\clocks{}}\rightharpoonup 2^{\{\lambda\}\cup\taactions{}_C}$ is a partial function over the states of $\mathcal{G}$ to a set of controllable actions (or a special nothing-symbol, $\tau$).
\end{definition}

\begin{definition}[Strategy Composition]
Given a TGA $\mathcal{G}=(\langle\locs,\loc_0,\taactions{},\clocks,\edges,\invars,\rangle,$ $\taactions_U,\taactions_C)$ and a memoryless strategy $\omega$, the composition $\mathcal{G}\|\omega$ provides a restriction of the transition-system of $\mathcal{G}$;
\begin{itemize}
	\item if $(\loc,\val)\trans{\alpha}(\loc',\val')$ then either we have $\alpha\in\Sigma^?$ or we have $\alpha\in\Sigma^!$ and $\alpha\not\in\taactions_C$ or $\alpha\in\omega(\loc,\val)$, and
	\item if $(\loc,\val)\trans{\delta}(\loc',\val')$  for $\delta\in\R$ then for all $0\leq \delta'<\delta$ it holds that $\lambda\in\omega(\loc,\val+\delta')$.
\end{itemize}
\end{definition}

Let $\varphi\subseteq\locs$ be a set of target locations for a TGA $\mathcal{G}$, then we can define a maximal set of winning states $\mathcal{W}$ as the maximal fix-point with;
\begin{itemize}
	 \item $\mathcal{W}_0=\{(\loc,\nu)\mid\loc\in\varphi\text{ and }\nu\in\mathbb{R}_{\geq_0}^{\clocks{}}\}$, and
	 \item $\mathcal{W}_n=\{(\loc,\nu)\mid\text{ for all }(\loc',\nu')\text{ where }(\loc,\nu)\underset{\mathcal{G}\|\omega}{\rightarrow}(\loc',\nu')\text{ we have }(\loc',\nu')\in\mathcal{W}_{n-1}\}$.
 \end{itemize}
% \todo[inline]{Definition of cooperative might not be needed, and same for the text below, other than the winning strategy}
\todo[inline]{remove fix-point notation}

A strategy is winning if $(\loc_0,\overset{\rightarrow}{0})\in\mathcal{W}$.

\todo[inline]{Preliminaries about UPPAAL, TIGA, Regions, Zones}
\fi


 % and we say that a strategy is co-operative winning if there exists $(\loc',\nu')\in\mathcal{W}$ s.t. $(\loc_0,\overset{\rightarrow}{0})\overset{\ast}{\rightarrow}(\loc',\nu')$.

% \end{definition}
% We say that a strategy $\omega$ i \emph{minimally co-operative} if it has the largest set of winning states $\mathcal{W}$ and it is co-operative winning.


% Let $\omega$ be a minimally co-operative strategy, then we call $\omega$ $k$-step if $\mathcal{W}^\omega_k=\mathcal{W}^\omega_{k+1}$.
% If all other minimally co-operative strategies are $k'$-step for $k'\geq k$ and not $k''$-step for $k''<k$, then we say that $\omega$ is \emph{step optimal}.
% Implicitly, a step optimal strategy ensures that after minimal help of the environment, the goal can surely be reached within $k$ transition firings.

% In a similar manner we can define a $t$-timed minimally co-operative strategy ensuring that the goal is reached within $t$ timeunits.
% Let $\xi=(\loc_0,\nu_0)\trans{\delta_0}(\loc_0,\nu'_0)\trans{\alpha_0}(\loc_1,\nu_1)\trans{\delta_1}\dots\trans{\alpha_n}(\loc_{n+1},\nu_{n+1})$ be a trace of the game $\mathcal{G}\|\omega$, then we let $\mathit{Sum}_\delta(\xi)=\sum_{0\leq i \leq n}\delta_i$ denote the total elapsed time for the given trace.
% Let $\Pi(\mathcal{G}\|\omega, s,s')$ denote the set of traces from $s,s'$, then a strategy $\omega$ is $t$-timed if for all $s,s'\in \mathcal{W}$ where $s'=(\loc,\nu)$ with $\loc\in\varphi$ we have that for all $\xi\in \Pi(\mathcal{G}\|\omega, s,s')$ it holds that $\mathit{Sum}_\delta(\xi)\leq t$.

% If all other minimally co-operative strategies are $t'$-timed for $t'\geq t$, but not $t''$-timed for $t''< t$, then we say that $\omega$ is \emph{timed optimal}.





==> Shield Synthesis for Timed Systems/experiments.tex <==
To validate our approach, we extend the case-study of Larsen et. al.~\cite{LarsenMT15} to a platoon of multiple cars\footnote{The source code, including some demonstrative videos and the running example used in the paper, is available online \cite{alexander_palmisano_2020_3903227}.}.
In the case study, an RL agent controls $n$ \emph{follower} vehicles in the platoon following an (environment controlled) \emph{leader} vehicle. 
All vehicles can drive a maximum of $20$m/s and have three different possible accelerations modes: $-2$m/s$^2$, $0$m/s$^2$ and $2$m/s$^2$ which can be changed at every time unit.
The goal of the RL agent is to control the followers in the platoon
such that the total distance between all vehicles is minimized.
Furthermore, the RL agent receives a negative reward if the distance between two cars is outside a safe region ($\leq 5$m) or is too large (above $200$m).
The hyper-parameters of the RL setting can be found in Appendix~\ref{app:RL}.
We used the models from~\cite{LarsenMT15} and synthesized timed post-shields with \uppaaltiga, as discussed in Sec.~\ref{sec:ts}.
We study the behaviour of RL agents in the context of 
\begin{enumerate*}
    \item no shielding,
    \item post-shielding during execution, and
    \item post-shielding during both training and execution.
\end{enumerate*}
We report the learning curves during the training phase and the performances in the execution phase for $n\in\{2,4,6,8,10\}$ where $n$ denotes the number of cars.
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1\linewidth]{images/training_plot_2.pdf}
		\caption{Results training phase.}
		\label{fig:result_training}
	\end{center}
	\vspace{-10pt}
\end{figure}


\emph{Training.}
%We trained controllers for 2, 4, 6, 8, and 10 cars, with and without a post-shield during training.
Each training episode starts with random but safe initial distances and velocities of all cars.
During the simulation, the environment picks the accelerations of the leading car via a uniform distribution. 
A training episode lasts for 2000 time units, or until the distance between two cars gets smaller than $5$m  or larger than $200$m. 
Note, that with a shield, a training episode always lasts $2000$ time units, since safety is always guaranteed.

Fig.~\ref{fig:result_training} compares the learning curves as a mean of $20$ training phases, for the unshielded case (left) and the shielded case (right). 
The reward in the unshielded case is considerably higher than in the shielded setting.
We observe that the agent exploits the relatively low risk of a crash and makes potentially unsafe choices.
Since the accelerations of the leading car are picked via an uniform distribution, it is unlikely, that e.g., the leading car accelerates to the maximum speed and then immediately hits the break until it reaches zero. 
Such risk tolerance is not allowed when deploying the shield as even a potential but unlikely future crash should be shielded against.
%
\emph{Execution Phase.}
%Next, we evaluated the performance and the safety of the resulting controllers, see Table~\ref{tab:results_execution}.
We tested all controller combinations for $1000$ simulations, and each simulation lasts until a crash or for a maximum of $2000$ time units.
%First, we report the results for the learned controllers that were trained without a shield and used without a shield in the execution phase. 
%We report the total number of crashes, the average number of time units per episode and the average total reward per simulation.
%Next, we took the same controllers again, but this time, we attached a shield in the execution phase and report the average reward.
%Finally, we give the results for the controllers, that were trained and exploited with a shield.
%Of course, in all shielded cases, the number of crashed was always zero and the number of time units per episode was 2000.
%Interestingly, we achieved better performance results, if we trained the controller without a shield, and then used the shield in the execution phase.
 Table~\ref{tab:results_execution} depicts the results. Note, that we learned a global controller for each number of cars (but use local shields) and that the controllers optimize a local minimum, therefore the controllers performances differ from each other.
Interestingly, we observe that the combination of unshielded training (Shield E) provides better results in our setting, compared to a RL agent utilizing the shield also during training (Shield T+E).
But more experiments are needed to discern this effect in more detail.


\begin{table}[tb]
\begin{center}
 \begin{tabular}{|c | c c c |c| c|}
\hline
&\multicolumn{3}{|c|}{No Shield} &\;Shield E\;&\;Shield T+E\;\\\hline
\;\#Cars\;&\;\#Crashes\;&\;Time\;&\;Reward\;&\;Reward\;&\;Reward\; \\\hline
2 & 703 & 1133 & 747 & 915 & 603 \\ \hline
4 & 13 & 1989 & 1070 & 685 & 393 \\ \hline
6 & 0 & 2000 & 638 & 617 & 375 \\ \hline
8 & 85 & 1908 & 477 & 495 & 386 \\ \hline
10 & 983 & 544 & 170 & 608 & 342 \\ \hline

\end{tabular}
  \caption{Results exploitation phase using 10000 simulations. 
  Number of crashes is given in absolute values over all simulations whereas Reward and Time measures are given as averages.
  Time and Crash values are omitted when shielding is applied as these are $>2000$ and 0 respectively. Time denotes the time-units of simulation prior to a first crash.}
  \label{tab:results_execution}
\end{center}
	\vspace{-0.5cm}
\end{table} 

==> Shield Synthesis for Timed Systems/faultmodels.tex <==


Since the shield only monitors the output of the implementation, after an error it has no information on what the system intended to do
and what state the system currently is in. It could be that e.g., (1) the output was wrong because of a transmission error and the
system  traversed according to one of the valid transitions, but the shield does not know which one, or (2) the output was a fluke and the
system did not change its state at all, or (3) that a deadline was missed by a delayed output, or (4) that a timer was erroneously reset.  
However, in order to be able to guide the current execution back to a state where the shield can end deviation and hand back control to the implementation,
the shields need ways of determining the current state of the implementation.
This idea is based on the assumption, that after the error the system behaves correctly again. Thus, if the shield and the system reach  the same state, it would be desirable for the system to take over.

In order to figure out the current state of the system, the erroneous transition leads to a different state in each fault model. Each one monitors one possible state the system could possibly be in after the fault. 
The fault models continue to monitor the behavior of the system during execution. 
As soon as a fault model can not follow the output of the implementation, it was not the correct fault model for the observed fault and
is discarded. 
Only if all active fault models agree on the state, we have presumably found the state the system is currently in.

\iffalse

In this paper, we focus on the location faults: go-to-any-location faults and go-to-next-location faults; and on the
clock faults:  wrong-reset faults and binary-swapped-clocks faults. We leave the discussion of the other fault models and their combination to future work. 

Each of the faults we consider induces a set of possible states the implementation could be in. We define the function
$\textrm{FM}(\A_\varphi):\locs{}_\varphi\times\posreals^{\clocks_\varphi}\rightarrow2^{\locs{}_\varphi\times\posreals^{\clocks_\varphi}}$ that computes the set of states to be monitored, for each type of fault we consider.

$\textrm{FM}(\A_\varphi, \loc_\varphi, \val_\varphi) :=$ \\
\begin{align}
 \{(\loc, \val_\varphi)\mid  & \loc\in\locs{}_\varphi \wedge \loc \neq \loc_\varphi \} \text{ for \emph{Go-to-any-location} faults.}\\
  \{(\loc, \val)\mid  & \loc\in\locs{}_\varphi \wedge \exists (\loc_\varphi, \val_\varphi) \xrightarrow{\oaction{a}}(\loc, \val)  \} \text{ for \emph{Go-to-next-location} faults.}\\
 \{(\loc_\varphi, \val)\mid & \exists x_i : \val(x_i)=0 \wedge \forall x_{j \neq i} : \val(x_j) = \val_\varphi(x_j) \}  \text{ for \emph{Wrong-reset} faults.}\\
\{(\loc_\varphi, \val)\mid  & \exists x_i,x_j : \val(x_i)=\val_\varphi(x_j), \val(x_j)=\val_\varphi(x_i) \wedge \\
& \forall x_{k \neq i,j}: \val(x_k) = \val_\varphi(x_k) \}   \text{ for \emph{Binary-swapped-clocks} faults.}
\end{align}
All of these fault types can be combined arbitrarily.
However, the more fault types that are used, the higher the complexity will be for the shield synthesis problem, as the set of states to be monitored grows larger.

For $(\loc_\varphi, \val_\varphi)$, we introduce a fault model for each state  $(l,v)\in\mutants(\A_\varphi, \loc_\varphi, \val_\varphi)$.
Each fault model corresponds to a copy of the specification automaton $\A_\varphi$, but uses $(l,v)$ as its initial state.



$\mutants(\A_\varphi, \loc_\varphi, \val_\varphi) =$ \\
\begin{align}
 \{(\loc, \val_\varphi)\mid  & \loc\in\locs{}_\varphi \wedge \loc \neq \loc_\varphi \} \cup\label{fault:gotoany}\\
  \{(\loc, \val)\mid  & \loc\in\locs{}_\varphi \wedge \exists (\loc_\varphi, \val_\varphi) \xrightarrow{\oaction{a}}(\loc, \val)  \} \cup\label{fault:gotonext}\\
 \{(\loc_\varphi, \val)\mid & \exists x_i : \val(x_i)=0 \wedge \forall x_{j \neq i} : \val(x_j) = \val_\varphi(x_j) \} \cup\label{fault:wrongresets}\\
\{(\loc_\varphi, \val)\mid  & \exists x_i,x_j : \val(x_i)=\val_\varphi(x_j), \val(x_j)=\val_\varphi(x_i) \wedge  \\
& \forall x_{k \neq i,j}: \val(x_k) = \val_\varphi(x_k) \} \label{fault:binaryswap}
\end{align}

 Line~\ref{fault:wrongresets} all {\em wrong reset} faults and Line~\ref{fault:binaryswap} all {\em binary swapped clocks} faults. For the illustrative example provided in Section~\ref{sec:demoex}, the corresponding numbers of fault models while in location $\textbf{l0}$ would be $2$, $1$, $1$ and $0$, respectively.
\fi


==> Shield Synthesis for Timed Systems/images/coordinator.tex <==
\begin{tikzpicture}[
every node/.style = {
		     shape=rectangle,% is not necessary, default node's shape is rectangle
                     draw=gray, very thick,
                     inner sep=.2cm,
                     rounded corners=3mm,
                     align=center,
                     font=\sffamily
}]

\node (unshielded) at (0,0) {\begin{tabular}{c}
Unshielded\\
$\N=\A_S$
\end{tabular}};

\node (shielded) at (6,0) {\begin{tabular}{c}
Shielded\\
$\N'=\A_S\|\A_F^0\|\dots \A_F^n$
\end{tabular}};

\path[->,thick,black] (-2,0) edge (unshielded);

\path[->,thick,black,bend left=30] (shielded) edge node[draw=none, below, yshift=0pt] {
\begin{tabular}{c}
Immediately when Equation~\ref{eq:allok} is true\\
Emit $\allok!$\\
let $q'=(s_S,s_1,\dots,s_n)$ be the state of the NTA $\N'$\\
$\N=\A_S$ with state $q=(s'_S)$ where $s_S\trans{\allok}s'_S$.
\end{tabular}
} (unshielded);

\path[->,thick,black,bend left=30] (unshielded) edge node[draw=none, above, yshift=0pt] {
\begin{tabular}{c}
Received $\startfm?$\\
let $q=(s_S)$ be the state of the NTA $\N$\\
let $\{s_0,\dots, s_n\}=\mutants(s_S)$\\
$\N'=\A_S\|\A_F^0\|\dots \A_F^n$ with $q'=(s_S,s_0,\dots,s_n)$.
\end{tabular}
} (shielded);

\end{tikzpicture}

==> Shield Synthesis for Timed Systems/images/shielded.tex <==
\begin{tikzpicture}[
every node/.style = {
		     shape=circle,% is not necessary, default node's shape is rectangle
                     draw=black, thin,
                     align=center,
                     minimum size=3mm
},xscale=0.7]



\begin{scope}[shift={(0,0)}]
\node (ol) at (0,0) {$\ell$};
\node (olo1) at (0,-3) {$\ell_{\alpha}$};
\node (old1) at (0,-6) {$\ell'$};
\node (ole) at (6,0) {$\ell_\tau$};


\path[->,thick,black,dashed] (ol) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\true,\alpha?,\emptyset)$} (olo1);
\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\psi,\overline{\alpha}!,X)$} (old1);

\path[->,thick,black] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-1cm] {$(\lastbound(\invars{}_\varphi(\ell)),\tau!,\emptyset)$}  (ole);

\end{scope}

\node[draw=none,font=\fontsize{30}{0}\selectfont] at (5.5,-3) {$\implies$};

\begin{scope}[shift={(10,0)}]
\node (ol) at (0,0) {$\ell$};
\node (olo1) at (0,-3) {$\ell_{\alpha}$};
\node (old1) at (0,-6) {$\ell'$};
\node (ole) at (7,0) {$\ell_\tau$};

\node (sl) at (7,-3) {$\overline{\loc}$};
\node (sle) at (7,-6) {$\overline{\loc'}$};

\path[->,thick,black,dashed] (ol) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\true,\alpha?,\emptyset)$} (olo1);
\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\psi,\overline{\alpha}!,X)$} (old1);

\path[->,thick,black] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-1cm] {$(\lastbound(\invars{}_\varphi(\ell)),\tau!,\emptyset)$}  (ole);

\path[->,thick,black] (sl) edge node[draw=none,sloped,pos=0.5,below,yshift=0.5cm]  {$(\psi,\overline{\alpha}!,X)$}  (sle);

\path[->,thick,black] (ole) edge node[draw=none,sloped,pos=0.5,below,yshift=.5cm]  {$(\true,\startfm!,\emptyset)$}  (sl);

\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,below,yshift=.4cm]  {$(\overline{\psi},\startfm!,\emptyset)$}  (sl);

\path[->,thick,black] (sl) edge node[draw=none,sloped,pos=0.5,below,yshift=.4cm]  {$(\true,\allok?,\emptyset)$} (ol);

\end{scope}
\end{tikzpicture}

==> Shield Synthesis for Timed Systems/images/violation.tex <==
\begin{tikzpicture}[
every node/.style = {
		     shape=circle,% is not necessary, default node's shape is rectangle
                     draw=black, thin,
                     align=center,
                     minimum size=3mm
},xscale=0.7]


\begin{scope}[shift={(0,0)}]
\node (ol) at (0,0) {$\ell$};

\node (oli1) at (-3,-6) {$\ell^1$};
\node[draw=none] at (-2,-6) {\dots};
\node (oli2) at (-1,-6) {$\ell^k$};
\node (olo1) at (1,-6) {$\ell^m$};
\node[draw=none] at (2,-6) {\dots};
\node (olo2) at (3,-6) {$\ell^n$};


\path[->,thick,black,bend right=30] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_1,\alpha_1?,X_1)$} (oli1);
\path[->,thick,black,bend right=10] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_k,\alpha_k?,X_k)$}  (oli2);
\path[->,thick,black,bend left=10] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_m,\alpha_m!,X_m)$} (olo1);
\path[->,thick,black,bend left=30] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_n,\alpha_n!,X_n)$}  (olo2);
\end{scope}

\node[draw=none,font=\fontsize{30}{0}\selectfont] at (5.5,-3) {$\implies$};

\begin{scope}[shift={(12,0)}]
\node (ol) at (0,0) {$\ell$};

\node (oli1) at (-4,-6) {$\ell^1$};
\node[draw=none] at (-3,-6) {\dots};
\node (oli2) at (-2,-6) {$\ell^k$};
\node (olo1) at (2,-3) {$\ell_{\alpha_m}$};
\node[draw=none] at (3,-3) {\dots};
\node (olo2) at (4,-3) {$\ell_{\alpha_n}$};

\node (old1) at (2,-6) {$\ell^m$};
\node[draw=none] at (3,-6) {\dots};
\node (old2) at (4,-6) {$\ell^n$};

\node (ole) at (0,-5) {$\ell_\tau$};

\path[->,thick,black,bend right=40,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_1,\alpha_1?,X_1)$} (oli1);
\path[->,thick,black,bend right=10,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_k,\alpha_k?,X_k)$}  (oli2);
\path[->,thick,black,bend left=10,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\true,\alpha_m?,\emptyset)$} (olo1);
\path[->,thick,black,bend left=40,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\true,\alpha_n?,\emptyset)$}  (olo2);
\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_m,\overline{\alpha_m}!,X_m)$} (old1);
\path[->,thick,black] (olo2) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_n,\overline{\alpha_n}!,X_n)$}  (old2);

\path[->,thick,black] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-1cm] {$(\lastbound(\invars{}_\varphi(\ell)),\tau!,\emptyset)$}  (ole);

\end{scope}
\end{tikzpicture}

==> Shield Synthesis for Timed Systems/intro.tex <==

Today's systems are becoming increasingly sophisticated and powerful. 
At the same time, systems have to perform highly safety critical tasks, e.g., in the
domain of self-driving cars, and make extensive use of machine learning, such as
reinforcement learning~\cite{FultonP19}.
As a result, complete offline verification %of such systems 
is rarely possible. 
This holds especially true for safety critical real-time systems, where a deadline violation comes with serious consequences.
%
An alternative is runtime verification~\cite{BlechFB12, BauerLS11, BartocciFBCDHJK19, BartocciFFR18}. % which aims to check the conformance of the system's executions w.r.t. some desired property.
Runtime enforcement  (RE)~\cite{KonighoferABHKT17, WuZW16, FalconeMFR11} extends this by enforcing the expected behavior of a system at runtime.

\begin{figure}
\captionsetup[subfigure]{font=footnotesize}
\centering
\subcaptionbox{Timed post-shielding}[.5\textwidth]{%
\begin{tikzpicture}
\definecolor{myblack}{cmyk}{.67,.33,0,.99}
\tikzstyle{box} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.7cm, text centered, draw=myblack]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{point} = [coordinate]
\definecolor{dgreen}{cmyk}{60, 0,100,0}

\node (system) [box, xshift=1.5cm] {$Sys$};
\node[inner sep=1pt, right of=system, xshift=2cm] (shield) {{{\includegraphics[bb= 15 10 800 780,scale=0.07]{images/shield-icon-blank.png}}}};

\draw[arrow, thick] (0,0) --  (system.west);
\draw[thick] (0.3,0) --  (0.3,-0.7);
\draw[arrow, thick] (0.3,-0.7) -- node [pos=0.75, above]{input} (3.8,-0.7);

\draw [arrow, thick] (system) -- node [anchor=south]{output} (shield);

\draw [arrow, thick] (4.6,-0.4) -- (6,-0.4);

\node[text width=1cm] at (4.45,-0.3) {$Sh$};
\node[text width=1cm] at (5.3,-0.4) {safe output};
\end{tikzpicture}}%
\subcaptionbox{Timed pre-shielding}
[.5\textwidth]{\begin{tikzpicture}
\definecolor{myblack}{cmyk}{.67,.33,0,.99}
\tikzstyle{box} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.7cm, text centered, draw=myblack]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{point} = [coordinate]
\definecolor{dgreen}{cmyk}{60, 0,100,0}

\node[inner sep=1pt, xshift=1.7 cm, yshift=0] (shield) {{{\includegraphics[bb= 15 10 800 780,scale=0.07]{images/shield-icon-blank.png}}}};
\node (system) [box, right of=shield, xshift=1.3cm, yshift=-0.3cm] {$Sys$};


\draw[arrow, thick] (0,-0.3) --  (0.8,-0.3);
\draw[thick] (0.3,-0.3) --  (0.3,-1.1);
\draw[thick] (0.3,-1.1) -- node [pos=0.75, above]{input} (2.8,-1.1);
\draw [thick] (2.8,-1.1) -- (2.8,-0.5);
\draw [arrow, thick] (2.8,-0.5) -- (3.25,-0.5);

\draw [arrow, thick] (1.8,-0.3) -- (system);

\draw [arrow, thick] (4.75,-0.3) -- node [pos=0.6, above]{output} (5.7,-0.3);

\node[text width=1cm] at (1.65,-0.3) {$Sh$};

\node[text width=1.1cm] at (2.6,0.2) {safe outputs};

\end{tikzpicture}}
\caption{Types of shielding.}
\label{fig:attach_shield}
\vspace{-5pt}
\end{figure}


In this paper, we focus on the enforcement of regular timed properties for reactive systems
and automatically synthesize \emph{timed shields} from \emph{timed automata} specifications.
A timed shield can be attached to a system in two alternative ways.
A \emph{timed post-shield} (see Fig.~\ref{fig:attach_shield}(a)) is implemented after the system.
It monitors the system and corrects the
system's output if necessary. A \emph{timed pre-shield} (see Fig.~\ref{fig:attach_shield}(b)) is placed before the system and provides a list of safe outputs to the system. This list restricts the choices of the system to safe actions. 

Timed post-shields guarantee the following two properties.
(1) \emph{Correctness:} the shielded system satisfies the safety specification, and
(2) \emph{No-Unnecessary-Deviation:}
the shield intervenes with the system only if safe system behavior would be
endangered otherwise. 
We extend timed post-shields to shields that additionally provide guarantees on the recovery time, after which control is handed back to the system; i.e., from that point on the shield forwards the outputs to the environment and does not deviate anymore.
(3a) \emph{Guaranteed-Recovery:}
the recovery phase ends within a \emph{finite time}, and
(3b) \emph{Guaranteed-Time-Bounded-Recovery:}
the recovery phase ends after a given \emph{bounded time}.

Timed pre-shields guarantee the following two properties.
(1) \emph{Correctness:} the shield provides only safe outputs to the system, and
(2) \emph{No-Unnecessary-Restriction:}
the shield provides all safe outputs to the system.

\iffalse
While basic timed post-shields are relatively simple and correct wrong system's outputs to arbitrary safe outputs, shields that give recovery guarantees need to consider all possible futures system executions after the fault.
We therefore introduce a notion of \emph{fault model} classes, a set of hypothesises of the state of the shielded system.
Each fault model is a hypothesis of the state of the system after a fault.% and monitors the system from that point on. 
If some system behavior cannot be explained by a specific fault model, it is discarded as the hypothesis is disproved.
We assume that at least one fault model correctly captures the behaviour of the system after the fault detection and will not be discarded. Once all active fault models agree on the state of the system with the shield, control can be given back to the system.
%, and control can be returned to the system, or (2) all fault models are disproved (or never agrees) and shielding continues indefinitely.
This construction comes with the price of an exponential overhead of the synthesis procedure compared with general post-shields.
%In this paper we show, how this approach reduces to solving a timed-safety game.
\fi

Shields can be employed during reinforcement learning (RL)
to ensure safety by enforcement both during a system's learning and execution phases~\cite{10.1007/978-3-319-11936-6_10,AlshiekhBEKNT18}. 
%In the traditional RL setting, in every time step, the learning agent chooses an action and sends it to the environment. 
%The environment evolves according to the action and sends the agent an observation of its state and a reward associated with the underlying transition. 
%The objective of the learning agent is to optimize the reward accumulated over this evolution.
We introduce a timed post-shield after the learning agent, as depicted in
Fig.~\ref{fig:attach_postposed_shield_learner}. 
The shield monitors the actions selected by the learning agent and corrects them if and only if the chosen action is unsafe.

To sum up, we make the following contributions:
\begin{itemize}
  \item We propose to synthesize timed shields from timed automata specifications.
  \item We discuss two basic types of timed shields: pre-shields and post-shields.
  \item We propose timed post-shields with the ability to recover.
  \item Our experiments show the potential of timed shields to enforce safety in RL.
\end{itemize}




\textbf{Related Work.}
%
In most work about RE, an enforcer monitors a program
that outputs events and can either terminate the program once it detects an error~\cite{Schneider00},
or alter the event in order to guarantee, for example, safety~\cite{HamlenMS06} or privacy~\cite{JiL17, WuRRLS18}.
Renard et al.~\cite{RenardFRJM19} and Falcone et al.~\cite{FalconeP19} considered RE for timed properties. The similarities between these enforcers and a shield is in
their ability to alter events. Their work only considers static programs whereas we consider enforcing correctness for reactive systems.
 
The term runtime assurance~\cite{Sha01} is often used if there exist 
a switching mechanism that alternates between running a high-performance system
and a provably safe one. These concept is similar to post-shielding, with the 
difference that we synthesize the entire provable safe system (the shield) including the switching mechanism while proving guarantees on recovery.

Könighofer et. al. introduced ~\cite{KonighoferABHKT17} shield synthesis from LTL specifications, which, while related, are not expressible enough to capture real time behavior and thus cannot shield against timing related faults in real timed systems.
Wu et al.~\cite{WuWDW19} extend shields for boolean signals to real-valued shields to enforce the safety of cyber-physical systems.
The concept of shield synthesis for RL from (probabilistic) LTL specification was discussed in~\cite{AlshiekhBEKNT18, abs-1807-06096} and early work on combining (basic) shielding with RL was demonstrated in~\cite{10.1007/978-3-319-11936-6_10}. 

We use the specification theory of Timed  In-put/Output Automaton (TIOA) used by \uppaalecdar~\cite{david2010ecdar}. 
To synthesize our timed shields we use \uppaaltiga~\cite{CassezDFLL05}, a tool which implements algorithms for solving games based on timed game automata with respect to reachability and safety properties, producing non-deterministic safety strategies. \uppaalstratego~\cite{DavidJLMT15, 10.1007/978-3-319-11936-6_10}
extends \uppaaltiga by the capability of optimizing these strategies with respect to desired performance measures.
While \uppaalstratego contains a RL component, we utilize a third-party, off-the-shelf, RL-system to demonstrate the applicability of the proposed method in a generic RL setting.

\textbf{Outline.} In Sec.~\ref{sec:def}
we give the formal notation and constructions.
Definition and construction of
timed post-shields (with recoverability garuantees under different fault models) are introduced in Sec.~\ref{sec:ts}  (Sec.~\ref{sec:tsg}). %along with constructions for shields with recoverability garuantees under different fault models.
Timed pre-shields are introduced in Sec.~\ref{sec:preempt}.
We discuss our experimental findings from a car platooning problem in Sec.~\ref{sec:exp} followed by a conclusion in Sec.~\ref{sec:conc}.



\begin{figure}[tb]
\centering
\begin{tikzpicture}
\definecolor{myblack}{cmyk}{.67,.33,0,.99}
\tikzstyle{box} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=0.9cm, text centered, draw=myblack]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{point} = [coordinate]
\definecolor{dgreen}{cmyk}{60, 0,100,0}

\node (env) [box] {Environment};
\node (la) [box, right of=env, xshift=3.4cm] {Learning Agent};

%\node (shield) [box, below of=la, yshift=-0.9cm] {Shield};



\node[inner sep=1pt, right of=env, xshift=3.8cm, yshift=-1.2cm] (shield) {{{\includegraphics[bb= 15 10 800 780,scale=0.07]{images/shield-icon-blank}}}};

\draw [arrow, thick] (env.5) -- node [anchor=south]{reward} (la.175);
\draw [arrow, thick] (env.-5) -- node [anchor=north]{~~observation} (la.185);

\draw [arrow, thick] (1.4, -0.1) |- node [anchor=south]{} (shield.175);

\draw [arrow, thick] (6,-2.3) -| node[pos=0.4, above] {safe action} (env);
\draw [arrow, thick] (6,-2.3) |- node[anchor=north] {} (la);

\draw [arrow, thick] (4.42, -0.5) -- node [anchor=west]{actions} (4.42, -0.95);
\node[text width=1cm] at (4.7,-1.5) {$Sh$};
\draw[thick] (4.42, -2.2) --  (4.42,-2.3);

\end{tikzpicture}
    \caption{A timed post-shield in a reinforcement learning setting.}
    \label{fig:attach_postposed_shield_learner}
\end{figure}

\iffalse
\textbf{OLD TEXT!}



%Runtime enforcement~\cite{re} is one of the technologies which provides a way for guaranteeing safety for systems which can otherwise not be verified. In runtime enforcement an \implementation is monitored during runtime, to check whether it satisfies certain properties. If a violation is detected, the monitor can intervene and correct the fault. Shield synthesis~\cite{shields} is a promising area of runtime verification. A shield is built according to a specification and receives the inputs from the environment and the outputs produced by the \implementation.
\begin{figure}
\begin{center}
\includegraphics[width=0.45\linewidth]{images/attach_shield.pdf}
\caption{Shielding a system.}
\label{fig:attach_shield}
\end{center}
\end{figure}





%If a fault is detected it is corrected by the shield and the shield takes over complete control of the outputs for a limited time span. Figure~\ref{fig:shield} illustrates the signal flow between the environment, the \implementation and the shield. It remains in control until it can guarantee that the implementation was guided back to a state, where its following behaviour will satisfy the current execution trace. As the \implementation might be way more refined than the shield, it is of high importance to hand back control as fast as possible. Thus, the two main challenges of a shield are to guarantee correctness for any \implementation and to ensure minimal deviation from the \implementation.



%The concrete approach for our timed shield synthesis will be as follows: Until a fault is observed, the shield simply receives the outputs of the \implementation and passes them on to the environment. If a fault is observed, we enter the shielded mode. In that mode, the shield has full control over all outputs, regardless of the behaviour of the \implementation. Additionally, we launch a set of fault models simulating the states the \implementation could have reached after the fault. These fault models will behave according to the outputs of the \implementation and will eventually converge in a single state. Meanwhile the shield will continue to correct the outputs of the \implementation, while searchig for a strategy that reaches the states of the fault models. If all fault models are in the same state as the shield, we are confident that the \implementation is in said state as well, and can hand back control.

%\begin{figure}
%\includegraphics[width=0.9\linewidth]{images/shield.png}
%\caption{Shielding an implementation.}
%\label{fig:shield}
%\end{figure}

The remainder of the paper is structured as follows:
first, we present a demonstrating example in Sec.~\ref{sec:demoex} and establish the preliminaries in Sec.~\ref{sec:def}.
Next, we discuss different classes of fault models for timed automata specifications in Sec.~\ref{sec:faults}.
Section~\ref{sec:shields} defines timed shields and proposes the synthesis algorithms for $t$-stabilizing and admissible shields. We present our experiments in Sec.~\ref{sec:exp} and conclude in Sec.~\ref{sec:conc}.

\fi

\iffalse

\section{Demonstrating example}
\label{sec:demoex}

\textbf{TODO: Rewrite this example, so that it shows all possible types of shielding:
Bofore, After, and the advantage of t-stabilizing shields}

In this section, we illustrate the challenges associated with shield synthesis for timed systems on a simple controller for a light switch.
Figure~\ref{fig:example_impl}(a) shows the specification automaton of the light switch: whenever the light is switched on,  this setting has to be kept for $1$ to $5$ time units,
and whenever the light is switched off, the light switch has to blink at least once every $3$ time units.
Note, that this is an abstract specification with loose timing constraints. The actual \implementation might turn of the light, if the movement in the room has ceased.

\begin{figure}

\minipage{0.49\textwidth}
\centering
  \includegraphics[width=0.7\linewidth]{images/spec.eps}
\endminipage\hfill
\minipage{0.49\textwidth}
\centering
  \includegraphics[width=0.7\linewidth]{images/impl}
\endminipage\hfill
\\
\minipage{0.49\textwidth}
\centering
  \includegraphics[width=0.7\linewidth]{images/FM1}
\endminipage\hfill
\minipage{0.49\textwidth}
\centering
  \includegraphics[width=0.7\linewidth]{images/FM2}
\endminipage\hfill

  \caption{Specification (a) and \implementation (b) and two fault models (c,d) of the light switch.}

\label{fig:example_impl}
\end{figure}


Next, lets consider a simple but faulty \implementation of the light switch as depicted in Figure~\ref{fig:example_impl}(b), where the red transition in the initial state shows the transient error that might appear.
After two steps, the faulty \implementation outputs an $\textbf{off!}$, without an initiating $\textbf{on?}$ signal.
Since this output would violate the specification, the shield has to interfere and to skip the $\textbf{off!}$ signal of the \implementation.

% \begin{figure}
% \minipage{0.24\textwidth}
  % \includegraphics[width=\linewidth]{images/FM1}
% \endminipage\hfill
% \minipage{0.24\textwidth}
  % \includegraphics[width=\linewidth]{images/FM2}
% \endminipage\hfill


  % \caption{Two fault models  of the light switch.}

% \label{fig:example_fms}
% \end{figure}


The tricky part is that the \implementation is considered as a black box and the shield can only observe the output of the \implementation.
Therefore, the shield has to produce an output trace, that is not only correct, but also leads the shield to a state in which the future signals
of the \implementation that are correct satisfy the specification again, such that the shield can hand back control to the \implementation.
In order to do that, the shield needs to align with the actual state of the \implementation after the fault.
In order to determine what that state might be, we launch several fault models that mimic the faulty \implementation. While the shield is active, these fault models are simulated according to the inputs and the outputs of the \implementation.
If a fault model can not follow the output of the \implementation, it was not the correct fault model for the observed fault and is discarded.
Only if all non-discarded fault models agree on the same state we can tell that the shield and the \implementation have synchronized again.

We give two possible fault models in Figure~\ref{fig:example_impl}(c,d). The first fault model assumes that the output was a fluke and that the \implementation is in location $\textbf{l0}$. The second one assumes that the fault led the \implementation to location $\textbf{l1}$.
 All our models are considered to be implicitly input-enabled, thus a missing input is simply ignored.

The slightly adapted specification and the fault models form a network of timed game automata. The shield is computed by playing a timed game on this network, with the goal of reaching the state of the fault models as fast as possible. The outputs of the shield, which are provided to the environment, are marked via an overline.

Table~\ref{tbl:example} shows a possible execution of the shielded faulty light switch.
After 2 time units a wrong output is produced, the shield corrects the output and all automata except the second fault model enter location $\textbf{l0}$ but with differing clock values. The shield corrects the output and immediately gives  a $\textbf{$\overline{blink}$!}$ output instead, which only changes the state of the shield itself.
After 1 time unit, the environment gives the input $\textbf{on?}$ and all automata enter the same location, but the first fault model with a different clock value.
The shield is still in control, but unless the \implementation gives an $\textbf{off!}$ signal, the most beneficial option for the shield is to wait, as this will synchronize the states.
After two seconds of waiting, the invariant of the first fault model is broken, and the fault model can be discarded.
At that point, all remaining fault models are in the same state as the shield, and we can hand back control to the actual \implementation.

\begin{table}
\centering
\begin{tabular}{ | c | c | c | c | c | c | } % c | c | }
 \hline
 timed trace  & init & (2,off!) & (0,$\overline{blink}$!)  & (1,on?) & (2, -) \\ \hline % (5,off!) | (5,off'!)
 Impl.  & (l0, x=0)  & (l0, x=0) & (l0, x=0)               & (l1, x=0)  & (l1, x=3) \\ % & (l0, x=0) \\
 Shield  & (l0, x=0) & (l0, x=2) & (l0, x=0)               & (l1, x=0)  & (l1, x=3) \\ % & (l0, x=0)  \\
 FM1  & -            & (l1, x=2) & (l1, x=2)               & (l1, x=3)  & \frownie{}  \\ %& x  \\
 FM2  & -            & (l0, x=2) & (l0, x=2)               & (l1, x=0)  & (l1, x=3) \\% & (l0, x=0)  \\
% FM3 & - & (l0, x=0) & (l1, x=0)  & (l1, x=3) \\% & (l0, x=0)  \\
 \hline
\end{tabular}
\caption{A possible shielded execution of the light switch.}
\label{tbl:example}
\end{table}

\fi



==> Shield Synthesis for Timed Systems/macros.tex <==
\newcommand{\ft}[1]{{\small\textsf{#1}}}

\newcommand{\opmod}{\textsc{OpenModelica}\xspace}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}



\newcommand{\actions}[1]{\ensuremath{\mathtt{A}_{#1}}}
\newcommand{\attActions}{\ensuremath{\actions{a}}}
\newcommand{\defActions}{\ensuremath{\actions{d}}}
\newcommand{\attAct}{\ensuremath{p_a}}
\newcommand{\defAct}{\ensuremath{p_d}}
\newcommand{\lang}[2]{\ensuremath{\mathcal{L}(#1,#2)}}
\newcommand{\langw}[2]{\ensuremath{\mathcal{L}^w(#1,#2)}}
\newcommand{\R}{\ensuremath{\mathbb{R_{\geq 0}}}}
\newcommand{\xdashrightarrow}[1]{\ensuremath{\overset{#1}{\dashrightarrow}}}
\newcommand{\attProf}{\ensuremath{\mu_{A}}}
\newcommand{\subf}{\ensuremath{\mathtt{Sub}}}
\newcommand{\prob}{\ensuremath{F}}
\newcommand{\probability}{\ensuremath{\mathbb{P}}}
\newcommand{\failueprob}{\ensuremath{\mathtt{Fail}}}
\newcommand{\denot}[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand{\true}{\ensuremath{\mathtt{tt}}}
\newcommand{\false}{\ensuremath{\mathtt{ff}}}
\newcommand{\aGraph}[1]{\ensuremath{\mathcal{G}^{#1}}}
\newcommand{\attSelect}{\ensuremath{\gamma_\attacker}}
\newcommand{\defSelect}{\ensuremath{\gamma_\defender}}
\newcommand{\attPosDelay}{\ensuremath{\Delta}}
\newcommand{\attDelay}{\ensuremath{\delta}}
\newcommand{\attSucc}{\ensuremath{{\mathtt{Env}}}}
\newcommand{\attFail}{\ensuremath{\delta_{f}}}

\newcommand{\astates}{\ensuremath{\mathsf{S}}}
\newcommand{\astate}[1][]{\ensuremath{{\mathsf{s}^{#1}}}}
\newcommand{\initastate}[1][]{\ensuremath{{\astate[#1]_{0}}}}
\newcommand{\finalvertices}{\ensuremath{F}}

\newcommand{\vvertices}{\ensuremath{\mathcal{V}^t}}
 \newcommand{\vvertex}[1][]{\ensuremath{{v^t_{#1}}}}
 \newcommand{\initvvertex}[1][]{\ensuremath{\vvertex[#1]^0}}
\newcommand{\vertices}{\ensuremath{\mathcal{V}}}

\newcommand{\vertex}[1][]{\ensuremath{{v_{#1}}}}
 \newcommand{\initvertex}[1][]{\ensuremath{\vertex[#1]^0}}
\newcommand{\initavertex}[1][]{\ensuremath{\vertex[#1]^{\attacker}}}
\newcommand{\adgvtoastates}{\ensuremath{M}}
\newcommand{\selectAttActions}{\ensuremath{Ac}}
\newcommand{\sdefender}{\ensuremath{\defender^\mathcal{S}}}
\newcommand{\sattacker}{\ensuremath{\mathcal{\attacker^S}}}
\newcommand{\tattacker}{\ensuremath{\mathcal{\attacker^\tau}}}
\newcommand{\environment}{\ensuremath{Env}}

\newcommand{\dm}[1]{\ensuremath{\mathop{}\!\mathrm{d} #1}}

\newcommand{\constraints}{\ensuremath{\mathcal{C}}}
\newcommand{\cconstraints}{\ensuremath{\mathcal{B}}}

\newcommand{\truns}{\ensuremath{\Omega^\tau}}
\newcommand{\dotrans}[2]{\ensuremath{[#1]^{#2}}}
\newcommand{\cost}{\ensuremath{\mathtt{C}}}
\newcommand{\costW}{\ensuremath{\mathtt{CW}}}
\newcommand{\satis}{\ensuremath{\vDash}}
\newcommand{\nsatis}{\ensuremath{\not\vDash}}

\newcommand{\expected}{\ensuremath{\mathbb{E}}}
\newcommand{\lowbounds}[1]{\ensuremath{\mathcal{B}^\geq(#1)}}
\newcommand{\upbounds}[1]{\ensuremath{\mathcal{B}^\leq(#1)}}
\newcommand{\initloc}[1][]{\ensuremath{\ell^{#1}_0}}
\newcommand{\loc}{\ensuremath{\ell}}
\newcommand{\sloc}{\overline{\loc}}
\newcommand{\uloc}{\hat{\loc}}
\newcommand{\comp}{\mathit{Comp}}
\newcommand{\taactions}{\ensuremath{\Sigma}}
\newcommand{\oactions}{\ensuremath{\Sigma_o}
}\newcommand{\iactions}{\ensuremath{\Sigma_i}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\vals}[1]{\mathcal{V}(#1)}
\newcommand{\valzero}{\val_0}
\newcommand{\oaction}[1]{\ensuremath{#1!}}
\newcommand{\iaction}[1]{\ensuremath{a?}}
\newcommand{\ltsover}[1][\adtree]{\ensuremath{\mathtt{LTS}(#1)}}
\newcommand{\graphover}[1][\adtree]{\ensuremath{\mathtt{Graph}(\adtree)}}
\newcommand{\intervals}{\ensuremath{\mathcal{B(\mathbb{R})}}}

\newcommand{\startfm}{\epsilon}
\newcommand{\allok}{\lambda}
\newcommand{\semof}[1]{{\llbracket#1\rrbracket}}
\newcommand{\lastbound}{{\mathit{LB}}}
\newcommand{\mutants}{\mathit{Mutants}}
\newcommand{\stateof}{\mathit{State}}
% TA
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\def\A{\ensuremath{\mathcal{A}}\xspace}
\def\Q{\ensuremath{\mathcal{Q}}\xspace}
\def\N{\ensuremath{\mathcal{N}}\xspace}
\def\G{\ensuremath{\mathcal{G}}\xspace}
\def\f{\ensuremath{\mathcal{f}}\xspace}
\newcommand\clocks[1][]{\ensuremath{{\mathit{X}_{#1}}}\xspace}
\newcommand\vclocks[1][]{\ensuremath{{\mathcal{X}^{\mathtt{V}}_{#1}}}\xspace}
\newcommand\tclocks[1][]{\ensuremath{{\mathcal{X}^{\mathtt{T}}_{#1}}}\xspace}
\newcommand\locs[1][]{\ensuremath{L_{#1}}\xspace}
\newcommand\invars[1][]{\ensuremath{I_{#1}}\xspace}
\newcommand\comitted{\ensuremath{K}\xspace}
\newcommand\posreals[0]{\ensuremath{\mathbb{R}_{\geq 0}}\xspace}
\newcommand\trans[1]{\ensuremath{\overset{#1}{\longrightarrow}}\xspace}
\newcommand\states[0]{\ensuremath{\mathcal{S}}\xspace}
\newcommand\guards[0]{\ensuremath{\mathcal{G}}\xspace}
\newcommand\reachable[0]{\ensuremath{\mathcal{R}}\xspace}
\newcommand\val[0]{\ensuremath{\nu}\xspace}
\newcommand\timed[0]{\ensuremath{\mathit{Time}}\xspace}
\newcommand\zones[0]{\ensuremath{\mathcal{Z}}\xspace}
\newcommand\updt[0]{\ensuremath{\mathcal{U}}\xspace}
% arrows
\newcommand{\overarrowi}[1]{\overset{#1}{\rightarrow}}
\newcommand{\overarrow}[1]{
  \mathchoice{\raisebox{-2pt}{ $\overarrowi{#1}$ }}
             {\raisebox{-2pt}{ $\overarrowi{#1}$ }}
             {\raisebox{-2pt}{ $\overarrowi{#1}$ }}
             {\raisebox{-2pt}{ $\overarrowi{#1}$ }}}
             
\newcommand{\longoverarrowi}[1]{\overset{#1}{\longrightarrow}}
\newcommand{\longoverarrow}[1]{
  \mathchoice{\raisebox{-3pt}{ $\longoverarrowi{#1}$ }}
             {\raisebox{-3pt}{ $\longoverarrowi{#1}$ }}
             {\raisebox{-3pt}{ $\longoverarrowi{#1}$ }}
             {\raisebox{-3pt}{ $\longoverarrowi{#1}$ }}}


\newcommand{\clockrates}{\ensuremath{\mathcal{R}}}
\newcommand{\pdf}{\ensuremath{\delta}}
\newcommand{\pmf}{\ensuremath{\gamma}}


\newcommand{\sattackers}{\ensuremath{\mathcal{S}}}

\newcommand{\edges}{\ensuremath{\mathit{E}}}
\newcommand{\dedges}{\ensuremath{\mathtt{E}_d}}
\newcommand{\reach}{\ensuremath{\mathtt{Reach}}}

\newcommand{\implementation}{implementation\xspace}
\newcommand{\implementations}{implementations\xspace}
\newcommand{\sys}{\uppProc{Sys}\xspace}
\newcommand{\spec}{\uppProc{Spec}\xspace}
\newcommand{\safe}{\uppProc{Safe}\xspace}
\newcommand{\env}{\uppProc{Env}\xspace}
\newcommand{\shield}{\uppProc{Ctr}\xspace}
\newcommand{\mspec}{\uppProc{mSpec}\xspace}
\newcommand{\specp}{\uppProc{Spec}'\xspace}
\newcommand{\mspecp}{\uppProc{mSpec}'\xspace}
\newcommand{\sh}{\uppProc{Sh}\xspace}
\newcommand{\shp}{\uppProc{Sh$_P$}\xspace}
\newcommand{\shs}{\uppProc{Sh$_S$}\xspace}
\newcommand{\shg}{\uppProc{Sh$_G$}\xspace}
\newcommand{\shgt}{\uppProc{Sh$_{GT}$}\xspace}

\newcommand{\fspec}{\uppProc{Spec$^{f}$}\xspace}
\newcommand{\fspecone}{\uppProc{Spec$^{f_1}$}\xspace}
\newcommand{\fspecn}{\uppProc{Spec$^{f_n}$}\xspace}
\newcommand{\fspeci}{\uppProc{Spec$^{f_i}$}\xspace}

\newcommand{\mfspec}{\uppProc{mSpec$^{f}$}\xspace}
\newcommand{\mfspecone}{\uppProc{mSpec$^{f_1}$}\xspace}
\newcommand{\mfspecn}{\uppProc{mSpec$^{f_n}$}\xspace}
\newcommand{\mfspeci}{\uppProc{mSpec$^{f_i}$}\xspace}

\newcommand{\wrm}{\uppProc{Wr}\xspace}
\newcommand{\act}{\uppProc{Act}\xspace}
\newcommand{\setact}{\uppProc{SetAct}\xspace}
\newcommand{\swr}{\mathcal{S}_{wr}\xspace}

==> Shield Synthesis for Timed Systems/postposed.tex <==
In  this section we will show how a safety strategy $\omega$ derived by either of the queries introduced in Section~\ref{sec:ts} can be used as a post-posed timed shield. In post-posed shielding, the shield is applied between the system under shielding and the environment (see Figure~\ref{fig:attach_shield} (a)). Every input and output of the system has to be provided to the shield, in order for the shield to check whether the outputs are safe and overwrite them in case they are not.
In the case of timed shields, additionally all timing constraints need to be observed, and in case an output is to be produced before a given deadline (marked by in invariant in the case of timed automata), the shield may interfere and produce that output at the last moment in time where it is expected, to ensure safety.


In order to use the  produced safety strategy $\omega$ as a shield, we simply need to compose it with the safety game $\mathcal{G}$. The composition $\mathcal{G}\|\omega$ will be a network of timed game automata where all unsafe transitions are pruned. 

Per construction of the component $\sh$, the outputs of the network will always conform to the outputs of the system, unless an error was detected or a timing constraint is about to be violated. Thus, an adapter that uses the network as a shield simply needs to simulate the network during execution of the system, and pass the outputs of the network on to the environment. 



%
% To use UPPAAL Stratego for the shielding, an adapter needs to be developed, that simulates all timed automata in $\mathcal{G}$ in parallel to the system under shielding and uses the strategy to suggest corrected outputs if needed. The intuition behind the adapter is given in Algorithm~\ref{alg:postposed}.
%
%
%\begin{algorithm}[H]
%	\SetAlgoLined
%	
%	\KwIn{Channels $in$, $out$, $out'$, Strategy $\omega$}
%	
%	\While{While true}{
%		\If{condition}{
%			instructions1\;
%			instructions2\;
%		}{
%			instructions3\;
%		}
%	}
%	\caption{How to write algorithms}
%	\label{alg:postposed}
%\end{algorithm}







$\alpha'\in\omega(\loc,\val)$

==> Shield Synthesis for Timed Systems/preempt.tex <==
In this section we define and construct timed pre-shields.
A timed pre-shield is attached before the system as illustrated in Figure~\ref{fig:attach_shield}(a).
At any point in time, a timed pre-shield provides \emph{a set of actions} \act
for the system to choose from.
This set of action can contain a delay action.
If this is the case, the system is permitted to wait without performing any discrete action. If the set does not include a delay action, the system has to produce an output immediately.
If the system picks the outputs according 
to this list, then it is guaranteed that the shield and the 
timed system together satisfy the specification.

\subsection{Definition of Timed Pre-Shields}

In this section we define timed pre-shields based on two properties;
correctness and no unnecessary restriction.

\begin{definition}[Correctness for Pre-Shields]
\label{def:corr_pre}
Let \spec be a specification, and let \sh be a pre-shield.
For any state $s$ from \sh, let \act$={\alpha_1,\dots,\alpha_n}$ be the set of enabled 
actions sent by \sh.
A pre-shield is correct, if it holds that if $\alpha$
is a wrong action for the given situation, then $\alpha\not\in\act$.
\end{definition}

\begin{definition}[No-Unnecessary-Restriction]
\label{def:mo_per}
Let \spec be a specification, and let \sh be a pre-shield.
For any state $s$ from \sh, let \act$={\alpha_1,\dots,\alpha_n}$ be the set of enabled 
actions sent by \sh.
A pre-shield is not unnecessarily restrictive, if it holds that if $\alpha$
is a correct action for the given situation, then $\alpha\in\act$.
\end{definition}

\begin{definition}[Timed Pre-Shields.]
Given a specification \spec. \sh is a timed pre-shield if it holds that \sh enforces correctness for any timed system \sys w.r.t. \spec (Def.~\ref{def:corr_pre}) and \sh is not unnecessarily restrictive (Def.~\ref{def:mo_per}).
\end{definition}
 
\subsection{Construction of Timed Pre-Shields}
%
We construct timed pre-shields according to the following algorithm.

\textbf{Algorithm 3.}
Starting from \spec, \mspec, we construct a timed pre-shield. 

\textbf{Step 1. Construction of the automaton \shield.} 
Since there is no concept of minimal deviation in pre-shields, the control options of the \shield component are not restricted. Instead, in this setting, we build \shield such that it can fire any output at any time, i.e., it has a single location and unguarded self-loops for every output. Note that timed pre-shields do not need primed outputs. 

 \textbf{Example.} \emph{The component \shield for the light switch is depicted in Fig.~\ref{fig:ctr_n}}. 
\begin{figure}[tb]
	
	%\minipage{0.89\textwidth}
	\centering
	\includegraphics[width=0.35\linewidth]{images/ctr_n-eps-converted-to.pdf}\\
	%(a)
	%\endminipage\hfill 
%	\\
%	\minipage{0.79\textwidth}
%	\centering
%	\includegraphics[width=0.99\linewidth]{images/mM1.eps}\\
%	(b)
%	\endminipage\hfill
	
	\caption{ The control options for a timed-pre shield of the light switch. }
	\label{fig:ctr_n}
	\vspace{-10pt}
\end{figure}

\textbf{Steps 2. Construct the timed safety game $\mathcal{G}$.}  
%
We construct the timed game $\mathcal{G}$ by the following composition:
$$\mathcal{G} = ~\mspec~|~\shield$$

\textbf{Step 3: Compute a strategy $\omega_{pre}$ of $\mathcal{G}$.}
%
Pre-shields ensure correctness (safety), i.e., 
the control objective is to ensure that \spec is
never violated. Solving the safety game w.r.t. the following query produces a strategy $\omega_{pre}$.
$$
\uppProp{control: A \Box~ \neg \mspec.\uppLoc{ERR}}
$$



\textbf{Step 4: Computing the set of enabled actions via zones.}
%
For a given state, the set of enabled actions \act is computed via zones.
From any given state, its zones can be calculated straightforwardly, see~\cite{alur1994theory}.
 %In case the current state is limited with an invariant, the last zone will have an upper bound, otherwise it will be unbounded.
\begin{figure}[tb]
\centering
\resizebox{0.38\textwidth}{!}{

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Grid [id:dp28127508069696305] 
\draw  [draw opacity=0] (100,32.33) -- (370.83,32.33) -- (370.83,272) -- (100,272) -- cycle ; \draw  [color={rgb, 255:red, 180; green, 180; blue, 180 }  ,draw opacity=1 ] (100,32.33) -- (100,272)(130,32.33) -- (130,272)(160,32.33) -- (160,272)(190,32.33) -- (190,272)(220,32.33) -- (220,272)(250,32.33) -- (250,272)(280,32.33) -- (280,272)(310,32.33) -- (310,272)(340,32.33) -- (340,272)(370,32.33) -- (370,272) ; \draw  [color={rgb, 255:red, 180; green, 180; blue, 180 }  ,draw opacity=1 ] (100,32.33) -- (370.83,32.33)(100,62.33) -- (370.83,62.33)(100,92.33) -- (370.83,92.33)(100,122.33) -- (370.83,122.33)(100,152.33) -- (370.83,152.33)(100,182.33) -- (370.83,182.33)(100,212.33) -- (370.83,212.33)(100,242.33) -- (370.83,242.33) ; \draw  [color={rgb, 255:red, 180; green, 180; blue, 180 }  ,draw opacity=1 ]  ;
%Shape: Rectangle [id:dp8127944690679545] 
\draw   (130,121.33) -- (250,121.33) -- (250,211.33) -- (130,211.33) -- cycle ;
%Shape: Rectangle [id:dp3762954793645883] 
\draw   (220,91.33) -- (340,91.33) -- (340,181.33) -- (220,181.33) -- cycle ;
%Straight Lines [id:da48357790251859556] 
\draw    (160,241.33) -- (370,32.33) ;
\draw [shift={(160,241.33)}, rotate = 315.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Shape: Brace [id:dp4129684908009801] 
\draw   (161.83,240.33) .. controls (165.08,243.69) and (168.38,243.75) .. (171.73,240.51) -- (174,238.32) .. controls (178.8,233.69) and (182.82,233.05) .. (186.06,236.41) .. controls (182.82,233.05) and (183.6,229.06) .. (188.39,224.43)(186.23,226.51) -- (190.66,222.23) .. controls (194.02,218.99) and (194.08,215.69) .. (190.84,212.34) ;
%Shape: Brace [id:dp9556890057520231] 
\draw   (219.83,181.33) .. controls (216.59,177.98) and (213.29,177.92) .. (209.94,181.17) -- (207.16,183.85) .. controls (202.37,188.48) and (198.35,189.12) .. (195.1,185.77) .. controls (198.35,189.12) and (197.57,193.12) .. (192.78,197.75)(194.94,195.67) -- (190,200.44) .. controls (186.65,203.68) and (186.59,206.98) .. (189.83,210.33) ;
%Shape: Brace [id:dp15127201365279008] 
\draw   (219.83,181.33) .. controls (223.13,184.63) and (226.43,184.63) .. (229.73,181.33) -- (232.71,178.35) .. controls (237.42,173.64) and (241.43,172.93) .. (244.73,176.23) .. controls (241.43,172.93) and (242.14,168.92) .. (246.85,164.21)(244.73,166.33) -- (249.83,161.23) .. controls (253.13,157.93) and (253.13,154.63) .. (249.83,151.33) ;
%Shape: Brace [id:dp09686810675940727] 
\draw   (309.83,91.33) .. controls (306.53,88.03) and (303.23,88.03) .. (299.93,91.33) -- (281.95,109.31) .. controls (277.24,114.02) and (273.23,114.73) .. (269.93,111.43) .. controls (273.23,114.73) and (272.52,118.74) .. (267.81,123.45)(269.93,121.33) -- (249.83,141.43) .. controls (246.53,144.73) and (246.53,148.03) .. (249.83,151.33) ;
%Shape: Brace [id:dp3982194514409336] 
\draw   (310,91) .. controls (313.21,94.39) and (316.51,94.47) .. (319.9,91.26) -- (338.48,73.63) .. controls (343.32,69.04) and (347.34,68.44) .. (350.55,71.83) .. controls (347.34,68.44) and (348.16,64.46) .. (352.99,59.87)(350.82,61.93) -- (371.58,42.23) .. controls (374.97,39.02) and (375.05,35.73) .. (371.84,32.34) ;
%Straight Lines [id:da04398142799293847] 
\draw    (101,272) -- (370.83,272.33) ;
\draw [shift={(372.83,272.33)}, rotate = 180.07] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da18796550398134126] 
\draw    (101,272) -- (100.01,34.33) ;
\draw [shift={(100,32.33)}, rotate = 449.76] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (82,33) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE y};
% Text Node
\draw (375,252) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE x};
% Text Node
\draw (133,102) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE a};
% Text Node
\draw (220,73) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE b};
% Text Node
\draw (187,234) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE z1};
% Text Node
\draw (178,170) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE z2};
% Text Node
\draw (253,165) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE z3};
% Text Node
\draw (252,95.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE z4};
% Text Node
\draw (353,68) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE z5};
% Text Node
\draw (140,233) node [anchor=north west][inner sep=0.75pt]   [align=left] {\LARGE S};


\end{tikzpicture}
}
\caption{The zones reachable by delay from a state $s$ in a TIOA with two clocks, \uppClock{x} and \uppClock{y}. The squares represent  constraints for two transitions with label \uppSync{a} and \uppSync{b}.}
\label{fig:regions}
\end{figure}

 \textbf{Example.} \emph{The concept of zones is illustrated in Fig.~\ref{fig:regions}, where the $X$ and $Y$ axis depict different clocks, and the squares represent the constraints in which different controllable actions $a$ and $b$ are enabled. We have for $a: \{1<x<5, 2<y<5\}$ and for $b: \{4<x<8, 3<y<6\}$}. %The zones are $z_1= \{x<3, y<2\};~ z_2 = \{3<x<4, 2<y<3\};~ z_3= \{4<x<5, 3<x<4\}; ~ z_4= \{5<x<7, 4<y<6\};$ and $z_5=\{x>7, y>6\}$}.


The set of enabled actions is kept up to date by monitoring the current state of $\sh_{pre}$.
 Whenever a new input or output from the system is received, the state is updated. From the new state, we calculate all zones that can be reached via delay and the actions enabled in each zone.  The set of actions \act for the current zone is sent to the system. In case the end of the zone is not met yet, this includes a delay action. If enough time passes so that the end of the current zone is met, the shield needs to check whether future zones permit actions. If so, the set of actions of the next zone is passed to the system. Otherwise, the current set of actions is transmitted again, this time without a delay action. The system may choose any of the permitted actions, including delay if possible.


 \textbf{Example.} \emph{In Fig.~\ref{fig:regions}, the actions enabled per zone are $z1=\{\}, z2=\{$\uppSync{a}$\}, z3=\{$\uppSync{a},\uppSync{b}$\}, z4=\{$\uppSync{b}$\}, z5=\{\}$. Thus, in the state $S$ which is in $z1$, \act is empty, after one time unit $\act=\{a\}$, and so on.} 

%For a given state in a (network of) timed automata it is straightforward to calculate a smallest enclosing zone.
%This straightforwardly yields us the set of zones that can be reached via delay and its enabled actions~\cite{alur1994theory}.

%This straightforwardly yields us the set of zones that can be reached via delay and its enabled actions~\cite{alur1994theory}.


\begin{theorem}
A shield $\sh_{pre}$ constructed according to Alg. 3 is a timed pre-shield.
\end{theorem}

\emph{Proof}. In order for $\sh_{pre}$ to be a timed pre-shield, $\sh_{pre}$ needs to satisfy correctness for pre-shields and the no-unnecessary-restriction property. $\sh_{pre}$ is correct, as the safety game removes every transition leaving the winning region. It has no-unnecessary-restriction, as \shield is not restricted when producing outputs, and all correct actions are kept when producing the strategy. \qed

\iffalse
\textbf{Discussion: timed pre-shields.} When using timed pre-shields, there is no concept of recovery or fault models, thus the computation is faster than the computation of shields with guaranteed recovery. Timed pre-shields are not as restricting to the system as post-shields, as instead of choosing one specific option and completely overruling the system, it provides the system with a choice of options. Thus, the overall efficiency of the system is kept as high as possible. 

Timed pre-shields can be specifically useful during the training (and employment) of machine learned controllers. It has already previously been shown~\cite{AlshiekhBEKNT18} that by removing unsafe options during learning, the learning process can be significantly speed up, and the learned controller will never chose unsafe options.
\fi

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\textbf{Discussion: Pre-shielding vs. Post-shielding.}
Post-Shielding has the advantage, that we treat the system as a total back box.
In order for pre-shielding to work, we need a system that chooses the actions
w.r.t. the suggestions of the shield. Usually, we have this setting in RL
where the shield can easily influence the set of available actions from the agent.
Instead of overruling the system, a pre-shield 
leaves the choice of which action should be executed always to the system, i.e.,
the system can do anything as long as it is safe. 
Thus, the overall efficiency of the system is kept as high as possible. 
It has already been shown that removing unsafe options during learning can significantly speed up the learning process~\cite{AlshiekhBEKNT18}.


% \begin{algorithm}[H]
	% \SetAlgoLined
	
	% \KwIn{Channels $in$, $out$, TGA Network \mathcal{G}||\omega$}
	% \KwOut{Map $L = \Phi \rightarrow\ \{ \mathcal{A} \}$}
	
	% $S = \{\initloc[0] .. \initloc[n]\}$
	
	% \While{While true}{
		% \If{condition}{
			% instructions1\;
			% instructions2\;
		% }{
			% instructions3\;
		% }
	% }
	% \caption{How to write algorithms}
 % \label{alg:pre}
% \end{algorithm}

==> Shield Synthesis for Timed Systems/ts.tex <==
This section defines and gives the construction of timed post-shields, illustrated in Fig.~\ref{fig:attach_shield}(a).
A timed post-shield is attached after the system, monitors its inputs and outputs, corrects the system's output if necessary and forwards the correct output to the environment. 

\subsection{Definition of Timed Post-Shields}

In this section, we define a timed post-shield based on its two desired
properties: %correctness, and no-unnecessary-deviation.

%The \textit{correctness} property  is the most important property of any post-shield. It states that the post-shield corrects any system's output such that a given safety specification is satisfied, i.e., the shielded system is guaranteed to be safe. 
%The \textit{no-unnecessary-deviation} property requires that if no fault was detected, the post-shield will not correct any of the systems outputs.


\begin{definition}[Correctness for Post-Shields.] \label{def:corr}
Let \spec be a specification, and let \sys be a timed system. We say that a shield
\sh ensures correctness if and only if it holds that 
$$(\sys~|~\sh)~ \leq \spec.$$
\end{definition}
%
That is, for any (faulty) system \sys, if it is placed in parallel with the shield, the shielded system is guaranteed to satisfy the specification. 



\begin{definition}[No-Unnecessary-Deviation.] \label{def:no_dev}
Let \spec be a specification, let \mspec be its corresponding monitor, let \sys be a timed system, and let \sh be a shield. 
%We denote by 
%$\textrm{out}$ and $\textrm{out'}$ timed sequences of outputs received from \sys and \sh, respectively.
%
%For any trace $\sigma$ produced by $(\env|\sys)$, we call $\sigma'$ the trace produced by $(\env|\sys|\sh)$ for the same set of delays and inputs. We say that \sh does not deviate from \sys unnecessarily if  for any $\sigma$ that does not lead \mspec to \uppLoc{ERR}, we have that for every output $o$ in $\sigma$, we have an output $o'$ in $\sigma'$ at the same point of time.
%
%Let $\sigma$ be any \emph{correct} timed trace of \sys, i.e., when monitoring $\sigma$ with \mspec the error state \mspec.\uppLoc{ERR} is never reached.  
Let $\sigma$ be any \emph{correct} timed trace of \sys, i.e., every action in $\sigma$ is correct, and no state along $\sigma$ is in $\swr$.  
We say that \sh does not deviate from \sys unnecessarily, if $(\sys|\sh)$ keeps the output for $\sigma$ intact.



%For any timed trace $\sigma$ produced by $(\env|\sys)$, we call $\sigma'$ the trace produced by $(\env|\sys|\sh)$ for the same set of delays and inputs. We say that \sh does not deviate from \sys unnecessarily if  for any $\sigma$ that does not lead \mspec to \uppLoc{ERR}, we have that for every output $o$ in $\sigma$, we have an output $o'$ in $\sigma'$ at the same point of time.

%We say that \sh does not deviate from \sys unnecessarily if 
%$$\neg \mspec.\uppLoc{ERR} \implies \textrm{out}(\sys) = \textrm{out}(\sh). $$
\end{definition}
In other words if \sys does not violate \spec, \sh simply forwards the outputs of \sys 
to the environment without altering them. Once we reach a state in $\swr$, there is no way to know whether the system would produce an output on time, and the shield is allowed to deviate.

\begin{definition}[Timed Post-Shields.]
Given a specification \spec, \sh is a timed post-shield if for any
timed system \sys, it holds that \sh enforces correctness of the shielded system 
w.r.t. \spec (Def.~\ref{def:corr}) and \sh does not deviate from \sys unnecessarily 
(Def.~\ref{def:no_dev}).
\end{definition}

\subsection{Construction of Timed Post-Shields}

In this section we discuss the synthesis procedure of timed post-shields without guarantees on the recovery time.

\textbf{Algorithm 1.} Let \spec be a specification, \mspec a monitor for \spec, and \sys a timed system.
We construct a timed post-shield \sh
via the following steps. 

\textbf{Step 1: Construction of the monitor \mspecp.}
To differentiate the outputs given by the system and those given by the shield, we prime the outputs of the shield. The monitor \mspecp is a copy of \mspec, where all outputs are primed. \mspecp is used to ensure that the outputs of the shield are correct.

\textbf{Step 2: Construction of the automaton \shield.}
The automaton \shield  is the only component that contains controllable transitions and depicts the control options for the shield, i.e., \shield produces the primed outputs. \shield is constructed such that the no-unnecessary-deviation property
is satisfied by the shield. 
Therefore, \mspec informs \shield whether the system's output is wrong or the current state is in $\swr$, i.e., the winning region of \mspec is left.
\shield can perform three types of actions: (1) \textit{pre-fault actions}: before an error was detected, \shield can only mirror actions produced by \sys; (2) \textit{post-fault actions}: after an error was detected, \shield has full control and can chose any action at a any time; and (3) \textit{last-chance actions}: whenever the current state is in $\swr$ and any delay would leave the winning region, the shield can prevent that possibility and can choose any action that is allowed in the current state of \mspecp.
%whenever an invariant in \spec is about to be violated, at the last point of time where the invariant still holds, the shield can prevent the possibility that \sys might violate the invariant and can choose any action that is allowed in the current state of \mspecp.

\begin{figure}[tb]
	\begin{center}
		\includegraphics[width=0.5\linewidth]{images/ctr-eps-converted-to.pdf}
		\caption{An automaton \shield,  defining control options of a shield for the light switch.}
		\label{fig:ex_shield}
	\end{center}
	\vspace{-10pt}
\end{figure}


\textbf{Example.} \emph{Fig.~\ref{fig:ex_shield} depicts the \shield component for the light switch of Fig.~\ref{fig:example_kim}(a). 
The two edges on the left (marked in blue) are pre-fault actions, that copy the system behaviour if no fault was detected, i.e., \uppGuard{error==0} (The error variable is set when \sys produces an output that would leave the winning region.).
The two transitions in the top right corner (green) are post-fault actions: if an error was detected, i.e., \uppGuard{error==1},  they will be enabled, and \shield can choose any output. 
The two transitions in the bottom
right (orange) show last-chance actions, for the case where the specification reached a time bound, in which case
\shield is allowed to take over, as a fault of the system may be imminent.}

\textbf{Step 3: Construct the timed safety game $\mathcal{G}$.}
We construct the timed game $\mathcal{G}$ by the following composition:
$$\mathcal{G} = ~\mspec~|~\mspecp~ |~\shield$$

In this game the monitor
\mspec observes whether the system \sys satisfies the specification \spec,
the monitor \mspecp observes whether the outputs of the shields are correct,
and \shield enforces that the shield does not deviate unnecessarily and is in charge of producing the primed outputs. 

\textbf{Step 4: Compute a strategy $\omega_S$ of $\mathcal{G}$.}
%
Post-shields ensure correctness (safety), i.e., 
the control objective is to ensure that \specp is
never violated by the shielded system. This can be expressed via the following safety 
query specifying that the error state should never be reached, given in \uppaaltiga syntax.
$$
\uppProp{control: A \Box~ \neg \mspecp.\uppLoc{ERR}}
$$

Solving the safety game w.r.t. this query produces a strategy $\omega_S$, which 
we use in the next step to produce a timed post-shield. 

\textbf{Step 5: Construction of the timed post-shield \shs.}
From the strategy $\omega_S$, we construct the shield \shs in the following way:
A shield \shs is the network of timed automata received by composing $\mathcal{G}$ with the derived strategy $\omega_S$, denoted by $\mathcal{G}\|\omega_S$, meaning that all unsafe transitions (or transitions that would not lead to recovery) are restricted. This shield may still permit multiple outputs in a given state, any of which ensures safety.



\begin{theorem}
A shield \shs constructed according to Alg. 1 is a timed post-shield.
\end{theorem}
\emph{Proof}. We have to proof that \shs satisfies the correctness property and the 
no-unnecessary-deviation property. 
\shs satisfies the correctness property, since all transitions %leading to $\uppProp{\mspecp.\uppLoc{ERR}}$ 
leaving the winning region were removed from $\mathcal{G}|\omega_S$. It thus holds that $(\sys~|~\sh)~ \leq \specp$.
Thus the primed outputs of the shield satisfy the specification.
Additionally, the construction $\mathcal{G}$ via the automaton \shield ensures that 
the shield cannot alter an action before a fault occurs, thereby ensuring that 
the shield cannot deviate unnecessarily \qed

%"!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

\section{Timed Post-Shields with Recovery Guarantees}
\label{sec:tsg}

In this section, we first discuss the challenges that we face when
synthesizing shields with the ability to recover from system faults
and discuss assumptions that we make on the system and its faults that are necessary for
our synthesis procedure.
Next, we define and construct timed post-shields with 
\textit{guaranteed recovery} and \textit{guaranteed time-bounded recovery}.

\subsection{Recovery under Fault Models}

In shield synthesis, we consider the system to be shielded as a black box,
which brings a huge scalability advantage, especially when shielding complex timed implementations.
Therefore, a shield has to ensure correctness for any system.

In order to end the recovery phase and to hand back control to the system, the shield
needs to \textit{resolve} the error that occurred, i.e., the state of the shield needs to align with the actual state of the system. The tricky part is, as mentioned before, that the system is considered as a black box and the shield can only observe the system's outputs but not its internal state.

In this paper we assume that the only violations that happen are due to {\em transient errors}. 
\begin{definition}[Transient Error]
A transient error is an error that happens only once, and has correct pre-error and post-error behavior.
\end{definition}
To determine the state of a system in case of a fault, we launch several \emph{fault models}
and assume that one of this fault models captures the fault.
%
\begin{figure}[tb]
	
	%\minipage{0.89\textwidth}
	\centering
	\includegraphics[width=0.85\linewidth]{images/M1-eps-converted-to.pdf}\\
	%(a)
	%\endminipage\hfill 
%	\\
%	\minipage{0.79\textwidth}
%	\centering
%	\includegraphics[width=0.99\linewidth]{images/mM1-eps-converted-to.pdf}\\
%	(b)
%	\endminipage\hfill
	
	\caption{A fault model \fspeci for a transient fault that captures an unexpected output that resets a clock. }
	\label{fig:fault}
\end{figure}
%
\begin{definition}[Fault Model]
Let \spec be a specification. A fault model \fspeci for \spec consists of two copies of the specification \spec, one copy for the pre-fault behavior and one copy for the
post-fault behavior. The two copies are connected with a single
transient error.
\end{definition}
\textbf{Example.} \emph{Fig.~\ref{fig:fault} gives an example of a fault model. 
The fault captures the situation, in which an \uppSync{off} signal is produced in the \uppLoc{OFF} location and this faulty signal additionally resets the clock \uppClock{xfm}, but does not change the location of the automaton. In the fault model,
this transient fault leads from the \uppLoc{OFF} location from the pre-fault 
part to the \uppLoc{OFF} in the post-fault part.}

Since we cannot observe the internal state of the system, 
we do not know which fault model captured the fault that occurred. 
Thus, the shield can only end the recovery phase if all fault models and the specification \textit{align}; i.e.,
if all \fspeci and \mspec reach the same state.
To achieve this, in the recovery phase, we monitor the behavior of the system and update the fault models accordingly.
If a fault model can not follow the output of the system (including not
allowing a delay that is possible in the system), it was not the
correct fault model for the observed fault and is discarded.
Only if all \emph{active}, i.e., non-discarded, fault models agree on the same state, 
the shield and the system synchronized again.

\textbf{Types of transient faults.}
We consider fault models covering the following fault types; categorized in location-faults, clock-faults, and their combination.
%
\begin{itemize}
\item{Location-faults:}
\begin{itemize}
\item{\emph{Go-to-any-location} faults:} the system goes to an arbitrary location.
To track the its location, we need a fault model for every location in \spec.
\item{\emph{Go-to-next-location} faults:} the system gives an incorrect output,
but continues in a correct successor location. Thus, the fault models only need to cover the valid successor locations.
\end{itemize}
\item{Clock-faults:}
\begin{itemize}
\item{\emph{Wrong-reset} faults:}  the system illegally resets a clock to zero.
Such faults occur, e.g., if  the system gives a planned reset at a wrong point in time, or the systems resets the wrong clock.
\item{\emph{Swapped-clocks} faults:} the system swaps the values of several selected clocks. This might be a {\em binary} swaps between two clocks, or {\em permutations} between several clocks.
\item{\emph{Missing-reset} faults:} the system ignores a planned reset of a clock, resulting in a clock value that is too high.
%\item{\emph{Arbitrary-value} faults:} the system sets one clock to an arbitrary (non-zero) value.
\end{itemize}
\end{itemize}

\textbf{Example.} \emph{The fault shown in Fig.~\ref{fig:fault}(a) is a wrong-reset fault, i.e., the fault does not change the location of the model, but only resets the clock \uppClock{xfm}.}

\subsection{Definition of Timed Post-Shields with Recovery Guarantees}

We now define shields which satisfy an additional property:  
\textit{guaranteed-recovery} or \textit{guaranteed-time-bounded-recovery}.

\textbf{The Guaranteed-Recovery Property.} 
%
In this paper, we synthesize shields with guaranteed (time-bounded) recovery 
under the assumption that the system satisfies the specification except for a single transient fault and that this fault is covered by one of the fault models \fspeci with $i\in \{1\dots n\}$.

\begin{definition}[Guaranteed Recovery]
Let \spec be a specification, let \mspec be its monitor, let $\text{\fspec}=\{\text{\fspecone}\dots\text{\fspecn}\}$ be a set of fault models, let \sys be a timed system with $\sys \leq$ \fspeci for some \fspeci $\in$ \fspec. We say that \sh guarantees recovery if for every trace $\sigma$ containing a single transient fault, i.e.,
there exists a point in time $t_1$ such that  \mspec reaches the error location \uppLoc{ERR} at $t_1$,
there exists a time $t_2>t_1$ such that after $t_2$ $(\sys | \sh)$ keeps $\sigma$ intact. 
\end{definition}
%
That is, if the system refines any of our considered fault models, we guarantee that an observed error will lead to recovery and the system and the shield give the same output again.  

\textbf{The Guaranteed-Time-Bounded-Recovery Property.} 
This property guarantees that the recovery phase lasts for at most $T$ time units
after a fault.

\begin{definition}[Guaranteed Time-Bounded Recovery]
Let \spec be a specification, let \mspec be its monitor, let $\text{\fspec}=\{\text{\fspecone}\dots\text{\fspecn}\}$ be a set of fault models, let \sys be a timed system with $\sys \leq$ \fspeci for some \fspeci $\in$ \fspec. We say that \sh guarantees recovery within a bound $T$ if for every trace $\sigma$ containing a single transient fault, i.e.,
there exists a point in time  $t_1$ such that  \mspec reaches the error location \uppLoc{ERR} at $t_1$,
we have that after time $t_1+T$, $(\sys | \sh)$ keeps $\sigma$ intact. 
\end{definition}
 

\subsection{Construction of Timed Post-Shields with Recovery Guarantees}

In this section we discuss the synthesis procedure of timed timed post-shields with 
\textit{guaranteed recovery} and with \textit{guaranteed time-bounded recovery}.

\textbf{Algorithm 2.} Let \spec be a specification, \mspec its monitor, 
and 
$\text{\fspec}=\{\text{\fspecone}\dots\text{\fspecn}\}$
a set of fault models.
Starting from \spec, \mspec, \fspec , we construct a timed post-shield 
with guaranteed-recovery (\shg), or 
with guaranteed-time-bounded-recovery (\shgt) via the following steps. 

\textbf{Steps 1 and 2.} Perform as in Section 3.2.

\textbf{Step 3: Construct the monitors \mfspeci}.
Transform the fault models \fspeci into monitors \mfspeci for $i\in \{1\dots n\}$.% in the same way the specification was transformed.

\textbf{Step 4: Construct the timed Game $\mathcal{G}$.}
%
Now we can consider the timed game given by the following composition:
%
$$\mathcal{G} = \text{\mfspecone}~|...|~\text{\mfspeci}~|~\mspec~|~\mspecp~ |~\shield$$
%
In this game, we observe conformance of the system with respect
to the fault models \mfspeci and the original specification via \mspec,
enforce the correctness of the shield via \mspecp, and ensure
no unnecessary deviations via \shield.
%
Next, we compute the winning strategies $\omega_g$ and $\omega_{gt}$ of $\mathcal{G}$ such that that the corresponding shields guarantee recovery and guarantee time-bounded recovery, respectively.

\textbf{Step 5a: Compute a strategy $\omega_g$ of $\mathcal{G}$ for guaranteed-recovery.}
%
For \emph{guaranteed recovery}, we need to establish a state where all
active %\footnote{A fault model is active, if its monitor is not in the \uppLoc{ERR} 	location} 
fault models agree with each other and the \specp, that is, they are all in the same location with same clock values. This can be achieved with the following leads-to property~\cite{behrmann2004tutorial}, specifying that if we observe a fault, this will eventually lead to recovery. 
\begin{align*}
	&\uppProp{control: A \Box~ \neg \mspecp.\uppLoc{ERR} \wedge \mspec.\uppLoc{ERR}~leadsto} \\ 
	&\uppProp{(\forall i. [\mspec^{f_i}.\uppLoc{ERR}~ \vee~ (\mspec^{f_i}.\uppVar{l} == \mspecp.\uppVar{l} ~\wedge
	~\mspec^{f_i}.\uppClock{x} = \mspecp.\uppClock{x})])}
\end{align*}

Solving $\mathcal{G}$ w.r.t. this query will produce a strategy $\omega_g$.
%
Note, that if a fault model is inactive, i.e., it reached its error-state, this means that \sys performed an output that was not valid in the fault model. 

\textbf{Step 5b: Compute a strategy $\omega_{gt}$ of $\mathcal{G}$ for guaranteed-time-bounded-recovery.}
%
We slightly change the  timed leads-to property to compute  $\omega_{gt}$
for guaranteed recovery within a time bound $T$:
\begin{align*}
	&\uppProp{control: A\Box~\neg \mspecp.\uppLoc{ERR} \wedge \mspec.\uppLoc{ERR} ~leadsto_{\leq T}} \\ 
	&(\forall i . [\mspec^{f_i}.\uppLoc{ERR} ~\vee~ (\mspec^{f_i}.\uppVar{l} == \mspecp.\uppVar{l} ~\wedge
	~\mspec^{f_i}.\uppClock{x} = \mspecp.\uppClock{x})])
\end{align*}
%
\textbf{Step 6: Construction of the timed post-shields \shg and \shgt.}
We construct a shield with guaranteed-recovery \shg by $\mathcal{G}\|\omega_g$,
and a shield with guaranteed-time-bounded-recovery \shgt by $\mathcal{G}\|\omega_{gt}$.


\begin{theorem}
The shields \shg and \shgt, constructed by Alg. 2, are timed post-shields with guaranteed-recovery and guaranteed-time-bounded-recovery, resp.
\end{theorem}
\emph{Proof.} Correctness and no-unnecessary-deviation are given as for regular timed post-shields. \shg (\shgt) is a shield with guaranteed-(time-bounded)-recovery, simply by the query it was produced from, which can only be satisfied if all traces in  \shg (\shgt) either do not encounter a fault, or the fault will lead to recovery at some point (within T time units) along the trace.  \qed






\textbf{Discussion: timed post-shields.}
Both types of shields, with and without recovery, have pros and cons.
Obviously, the ability of guaranteed recovery after a system fault is highly desirable.
This is especially true, if the system to be shielded is highly optimized and
performs complex tasks that are not captured in the specification of the shield.
Nevertheless, it may not be feasible to synthesize post-shields with the ability to recover.
First, guaranteed recovery is not always possible and therefore, no shield that guarantees recovery may exist. An obvious example that demonstrates this fact is a shield for a system that never resets one of its clocks. If a fault occurred that changes the value of this clock, synchronization is never possible. 
Second, to capture any transient fault that is possible under a given fault category, an exponential number of fault models is needed. This results in an exponential blowup in the state space and synthesis time. Therefore, it may not be feasible to synthesize
shields with guaranteed recovery for large specifications considering a large number of fault models. %The construction of post-shields without recovery has linear complexity
%and therefore, these shields are also suitable to shield against large specifications.

%Solving any of these queries on the timed game $\mathcal{G}$ will produce a memoryless strategy $\omega$, collecting a set of permitted actions for each state. A %strategy can be turned into a post-posed or preemtive timed shield $Sh$, which will be discussed in Sections~\ref{sec:postposed} and ~\ref{sec:preempt}, %respectively.


\iffalse
\textbf{before tina touched it}
\subsection{Producing a Timed Post-Shield}
\label{sec:convert}

We now will discuss the transformation of a strategy $\omega_{p}$, $\omega_{g}$ or $\omega_{gt}$, into a pure safety shield, a timed shield with guaranteed recovery, and a timed shield with guaranteed time-bounded recovery, respectively.

A shield is derived from the safety game $\mathcal{G}$, which is a network of timed game automata $\mathcal{G} = \mspec~|~\mspecp~ |~\shield$ in the case of pure safety, and $\mathcal{G} = ~\mspec^{f1}~|...|~\mspec^{fn}~|~\mspec~|~\mspecp~ |~\shield$ in the case of a shield with guaranteed recovery.

\begin{definition}
A shield $Sh$ is the network of timed automata received by composing $\mathcal{G}$ with the derived strategy $\omega$, denoted by $\mathcal{G}\|\omega$, meaning that all unsafe transitions (or transitions that would not lead to recovery) are restricted.
\end{definition}

A shield can be applied after any system, shielding its outputs towards the environment.

Independently on the used type of shield, the following theorem holds for any shield $Sh$ derived this way:

\begin{theorem}
$$(\sys~|~\sh)~ \leq \specp$$
\end{theorem}

That is, for any system \sys, regardless of which fault(s) it contains, if it is placed in parallel with the shield, we will guarantee that it satisfies the specification. 

In addition, we guarantee that we only interfere with the system, in case a fault was detected. We denote by $\textrm{out}$ the timed sequence of outputs received from $\sys$ and by $\textrm{out'}$ the timed sequence of outputs produced by the shield.

\begin{theorem}
$$\neg \mspec.\uppLoc{ERR} \implies \textrm{out} = \textrm{out'} $$
\end{theorem}


Finally, if $Sh$ is a shield with guaranteed (time-bounded) recovery, we have that:
\begin{theorem}
	$$ \exists n : \sys \leq \spec^{fn} \implies (\sys~|~Sh~) \leq \specp \wedge \mspec.\uppLoc{ERR}~\uppProp{leadsto}_{(\leq T)} \textrm{recovery}$$
\end{theorem}

That is, if the system refines any of our considered fault models, in addition to guaranteeing safety, we guarantee that an observed error will lead to recovery (within the time bound \uppVar{T}), where recovery means that all active fault models will be in the same state as the specification. 

\textbf{Discussion: timed post-shields with/without guaranteed (time - bounded) recovery.}
Both types of shields, with and without recovery, have pros and cons.
Obviously, the ability of guaranteed recovery after a system fault is highly desirable.
This is especially true, if the system to be shielded is highly optimized and
performs complex tasks that are not captured in the specification of the shield.
Nevertheless, it may not be feasible to synthesize post-shields with the ability to recover for one of two reasons.
First, guaranteed recovery is not always possible and therefore, no shield that guarantees recovery exists. An obvious example that demonstrates this fact is a shield for a system that never resets one of its clocks. If a fault occurred that changes the value of this clock, synchronization is never possible. 
Second, to capture any transient fault under a given fault category that is possible, an exponential number of fault models is needed. This results in an exponential blowup in the state space and in the synthesis time. Therefore, it may not be traceable to synthesize
shields with guaranteed recovery for large specifications considering a large number of fault models. The construction of post-shields without recovery has linear complexity
and therefore, these shields are also suitable to shield against large specifications.
\fi

%\subsection{Fault models}
%\input{faultmodels}

% \subsection{Generating shields in UPPAAL Stratego}
% \todo{probably not needed}

% In this section we show how t-stabilizing shields can be produced in UPPAAL Stratego. This will be demonstrated on the example already shown in Figure~\ref{fig:example_kim} and ~\ref{fig:ex_shield}.

% To make the approach work in UPPAAL, we need to produce a monitor that constantly checks whether the system has recovered, by checking whether the conditions for recovery is met and setting an according flag in case. The condition for recovery is that for each fault model either the fault model is inactive, or it is in the same state as the specification. Since guards in UPPAAL do not permit disjunction, the monitor contains several transitions containing the different cases. Only two of these transitions are illustrated in Figure~\ref{todo}.

% The final query used to synthesize a shield with guaranteed time-bounded recovery is given below. It is a rewritten, yet equal, form of the query to the one presented earlier.
% \begin{align*}
% \textrm{strategy REC = }& \textrm{control: } A[]  \textrm{not mSpecp.ERR and} \\ 
% &(( \textrm{not mSpec.ERR})  \textrm{ or } t<=T  \textrm{ or recovered})
% \end{align*}
% This will produce a safety strategy, which can then be exported and used as a shield. The format of the exported strategy is a list of reachable states with a set of attached (sometimes time-guarded) actions that are permitted in the given state, including the option to delay, if it is permitted by the invariants and allowed by the strategy. An extract showing a (slightly simplified) example of the output is shown below:

% \begin{align*}
% \textrm{State:} & ( \textrm{mSpec.ERR mSpecp.ON ... ) error=1 recovered=0 states=1 ...} \\
% & \textrm{When (1 \textless=xs \&\& xs\textless=5), Shield.\_id7-\textgreater Shield.\_id7 \{ error == 1, off\_p!, 1 \}} \\
% &\textrm{mSpecp.ON-\textgreater mSpecp.OFF \{ xs \textgreater= 1, off\_p?, xs := 0, states := 0 \}}\\
% &\textrm{While you are in	(xs\textless 1), wait.}
% \end{align*}


% A complete UPPAAL model containing four fault models and all needed components is available online~\footnote{TODO: upload and add link}. The calculation of a timed shield with guaranteed time-bounded recovery for that example took $9.6$ seconds. This is, admittedly, a very long time for this very small example, and proofs the argument we made earlier, that guaranteed time-bounded recovery is only suitable for the most critical components in larger systems, and cannot be applied to the complete system at once. Comparatively, producing a timed shield with only guaranteed recovery only takes $0.004$ seconds (after pruning the fault models from the UPPAAL model, as they are not used for the pure safety game). 




%
%\section{Demonstrating example}
%\label{sec:demoex}
%
%In this section, we illustrate the challenges associated with shield synthesis
%for timed systems on a simple controller for a light switch.
%Figure~\ref{fig:example_impl}(a) shows the environment, which might randomly
%turn the light on, and receives the on and blink signal from the shield.
%Figure~\ref{fig:example_impl}(b) shows the specification automaton of the light
%switch: whenever the light is switched on,  this setting has to be kept for $1$
%to $5$ time units, and whenever the light is switched off, the light switch has
%to blink at least once every $3$ time units.
%Note, that this is an abstract specification with loose timing constraints. The
%actual \implementation might turn of the light, if the movement in the room has
%ceased.
%
%\begin{figure}
%	
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/spec.eps}
%	% \endminipage\hfill
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/impl}
%	% \endminipage\hfill
%	% \\
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/FM1}
%	% \endminipage\hfill
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/FM2}
%	% \endminipage\hfill
%	
%	% \caption{Specification (a) and \implementation (b) and two fault models
%	%(c,d) of the light switch.}
%	\includegraphics[width=0.99\linewidth]{images/shield_ex.png}
%	\caption{Environment (a), Specification (b), two possible faulty
%		implementations(c,d) and four fault models (e,f,g,h) of the light switch.}
%	\label{fig:example_impl}
%\end{figure}
%
%
%Next, lets consider a simple but faulty \implementation of the light switch as
%depicted in Figure~\ref{fig:example_impl}(c), where the red transition in the
%initial state shows the transient error that might appear.
%After two steps, the faulty \implementation outputs an $\textbf{off!}$, without
%an initiating $\textbf{on?}$ signal.
%Since this output would violate the specification, the shield has to interfere
%and to skip the $\textbf{off!}$ signal of the \implementation.
%
%% \begin{figure}
%% \minipage{0.24\textwidth}
%% \includegraphics[width=\linewidth]{images/FM1}
%% \endminipage\hfill
%% \minipage{0.24\textwidth}
%% \includegraphics[width=\linewidth]{images/FM2}
%% \endminipage\hfill
%
%
%% \caption{Two fault models  of the light switch.}
%
%% \label{fig:example_fms}
%% \end{figure}
%
%
%
%The goal of the shield is to produce an output trace, that is not only correct,
%but also leads the shield to a state in which the future signals
%of the \implementation that are correct satisfy the specification again, such
%that the shield can hand back control to the \implementation.
%In order to do that, the shield needs to align with the actual state of the
%\implementation after the fault. The tricky part is that the \implementation is
%considered as a black box and the shield can only observe the output of the
%\implementation.
%In order to determine what that state might be, we launch several fault models,
%assuming that one of them mimics the faulty \implementation. While the shield is
%active, these fault models are simulated according to the inputs and the outputs
%of the \implementation.
%If a fault model can not follow the output of the \implementation (including not
%allowing a delay that is possible in the \implementation), it was not the
%correct fault model for the observed fault and is discarded.
%Only if all non-discarded fault models agree on the same state and the shield
%has reached that state as well, can we tell that the shield and the
%\implementation have synchronized again.
%
%We give four possible fault models in Figure~\ref{fig:example_impl}(e,f,g,h).
%The first fault model assumes that the output happened and reset the clock, but
%that the \implementation still is in location $\textbf{OFF}$. The second one
%assumes that the fault led the \implementation to location $\textbf{ON}$,
%reseting the clock. The next two fault models are the same, but without reseting
%the clock. 
%
%The slightly adapted specification and the fault models form a network of timed
%game automata. The shield is computed by playing a timed game on this network,
%with the goal of reaching the state of the fault models as fast as possible. The
%outputs of the shield, which are provided to the environment, are marked via an
%overline.
%
%Table~\ref{tbl:example} shows a possible execution of the shielded faulty light
%switch.
%After 2 time units a wrong output is produced, the shield corrects the output
%and all automata, except the second and fourth fault model, enter location
%$\textbf{OFF}$ but with differing clock values. The shield corrects the output
%and immediately gives  a $\textbf{$\overline{blink}$!}$ output instead, which
%only changes the state of the shield itself.
%After $1$ time unit, the environment gives the input $\textbf{on?}$ and all
%automata enter the same location, but fault models $2$ and $4$ have a different
%clock value.
%The shield is still in control, but unless the \implementation gives an
%$\textbf{off!}$ signal, the most beneficial option for the shield is to wait for
%that signal, in order to follow it.
%After two seconds of waiting, the invariant of fault model $4$ is broken, and
%the fault model can be discarded.
%As soon as the \implementation sends the $\textbf{off!}$ signal, all remaining
%fault models are in the same state and the shield can follow them by creating
%the $\textbf{$\overline{off}$!}$ output. Now all automata are aligned and we can
%hand back control to the actual \implementation.
%
%\begin{table}
%	\centering
%	\begin{tabular}{ | c | c | c | c | c | c |  c | }
%		\hline
%		timed trace  & init & (2,off!) & (0,$\overline{blink}$!)  & (1,on?)    & (3,
%		off!) & (0, $\overline{off}$!) \\ \hline % (5,off!) | (5,off'!)
%		Impl.1  & (OFF, x=0) & (OFF, x=0) & (OFF, x=0)            & (ON, x=0)  & (OFF,
%		x=0)  & (OFF, x=0) \\ % & (l0, x=0) \\
%		Shield  & (OFF, x=0) & (OFF, x=2) & (OFF, x=0)            & (ON, x=0)  & (ON,
%		x=3)   & (OFF, x=0) \\ % & (l0, x=0)  \\
%		FM1  & -             & (OFF, x=0) & (OFF, x=0)            & (ON, x=0)  & (OFF,
%		x=0)  & (OFF, x=0)  \\ %& x  \\
%		FM2  & -             & (ON, x=0)  & (ON, x=0)             & (ON, x=1)  & (OFF,
%		x=0)  & (OFF, x=0) \\% & (l0, x=0)  \\
%		FM3 & - 			  & (OFF, x=2) & (OFF, x=2)            & (ON, x=0)  & (OFF, x=0)  &
%		(OFF, x=0)\\
%		FM4 & -              & (ON, x=2)  & (ON, x=2)             & (ON, x=3)  &
%		\frownie{}  & \frownie{}\\% & (l0, x=0)  \\
%		
%		\hline
%	\end{tabular}
%	\caption{A possible shielded execution of the light switch with the faulty
%		\implementation $1$.}
%	\label{tbl:example}
%\end{table}
%
%Table~\ref{tbl:example2} shows a possible execution, where we assume the
%\implementation behaved like faulty \implementation $2$. The fault models are
%again initialized after a two second delay followed by the faulty
%$\textbf{off!}$ signal. Assuming that we do not receive an $\textbf{on?}$
%signal, the shield could simply loop with $\textbf{blink!}$ signals, and wait
%for all other models to collect in the $\textbf{OFF}$ location, thus, let us
%assume after one second an $\textbf{on?}$ signal arrives. While all automata are
%in the same location, there is a one second delay between the shield and the
%\implementation. This means that the \implementation can leave the location with
%an $\textbf{off!}$ signal one second earlier than the shield can follow. As soon
%as the shield follows it with an $\textbf{$\overline{off}$!}$ signal, the
%\implementation can already move back to the \textbf{ON}$ state, and the shield
%will never be able to catch up. Thus, in this case no t-stabilizing shield can
%exist, and unless the environment helps us at some point by delaying the
%\textbf{on?}$ signal long enough for the shield to wait the \implementation in
%the $OFF$ location, we will not be able to give back control.
%
%\begin{table}
%	\centering
%	\begin{tabular}{ | c | c | c | c | c | c |  c  | }
%		\hline
%		timed trace  & init & (2,off!)     & (1,on?)    & (1, off!) & (1,
%		$\overline{off}$!) & ... \\ \hline % (5,off!) | (5,off'!)
%		Impl.2  & (OFF, x=0) & (ON, x=0)   & (ON, x=1)  & (OFF, x=0)  & (OFF, x=1) &
%		... \\ % & (l0, x=0) \\
%		Shield  & (OFF, x=0) & (OFF, x=2)  & (ON, x=0)  & (ON, x=1)   & (OFF, x=0) &
%		... \\ % & (l0, x=0)  \\
%		FM1  & -             & (OFF, x=0)  & (ON, x=0)  & \frownie{}  & \frownie{} &
%		...  \\ %& x  \\
%		FM2  & -             & (ON, x=0)   & (ON, x=1)  & (OFF, x=0)  & (OFF, x=1) &
%		... \\% & (l0, x=0)  \\
%		FM3 & - 			  & (OFF, x=2)  & (ON, x=0)  & \frownie{}  & \frownie{} & ...\\
%		FM4 & -              & (ON, x=2)   & (ON, x=3)  & (OFF, x=0)  & (OFF, x=1) &
%		...\\% & (l0, x=0)  \\
%		
%		\hline
%	\end{tabular}
%	\caption{A possible shielded execution of the light switch with the faulty
%		\implementation $2$.}
%	\label{tbl:example2}
%\end{table}
%
%
%\section{Timed Shields}
%
%In this section we will propose algorithms for the generation of three types of
%shields, a general shield that only cares about satisfying the specification,
%and two more advanced shields that rely on fault models in order to determine
%when / if they can give back control to the shielded controller. For that we
%assume a set of fault models $M_n$, and a safety specification $Spec$. 
%
%\subsection{General Timed Shields}
%
%General timed shields are a basic form of runtime enforcement, as they do not
%take over control for a given time, but simply overwrite any outputs that do not
%satisfy the specification. This means, they symbolize the most permissive
%strategy~\ref{test} of the system, that satisfies the specification.
%
%\begin{definition}[General timed shields]
%	A general timed shield $X_g$, is the most permissive refinement of $Spec$, i.e.,
%	$X_g \leq_{mp} Spec$.
%\end{definition}
%
%The advantage of general timed shields is that they need less information about
%the actual implementation or possible faults. This makes them very usable for
%the shielding of controllers that were derived via machine learning. 
%
%\subsection{Admissible Timed Shields}
%
%Admissible timed shields use the fault models in order to determine when control
%can be given back to the controller. They will shield the system until all
%(non-discarded) fault models are in the same state as the shield. However, there
%is no guarantee for this to ever happen, and some cooperation from the
%environment might be necessary to achieve it.
%
%\begin{definition}[Admissible timed shields]
%	An admissible timed shield is the component $X_{ad}$, so that $(M_1 || M_2 ||
%	... || M_n || X_{ad}) \leq_{mp} Spec$ and \textbf{$\overline{o}$!}$ ==
%	\textbf{o!}$ whenever $state(M_1) == state(M_2) == ... == state(M_n) ==
%	state(X_{ad})$.
%\end{definition}
%
%Admissible shields are to be used, when the considered fault models are not
%synchronizing timed automata. In most practical cases, the environment will not
%actively try to keep the automata from synchronizing, thus, the shield will most
%likely have a chance of aligning its state with the implementation eventually. 
%
%\subsection{T-stabilizing Timed Shields}
%
%T-stabilizing timed shields guarantee to give back control within t-timesteps.
%They will shield the system until all (non-discarded) fault models are in the
%same state as the shield, but never longer than for $t$ time units in a row. 
%
%\begin{definition}[T-stabilizing timed shields]
%	A t-stabilizing timed shield is the component $X_{ts}$, so that $(M_1 || M_2 ||
%	... || M_n || X_{ts}) \leq_{mp} Spec$, \textbf{$\overline{o}$!}$ == \textbf{o!}$
%	whenever $state(M_1) == state(M_2) == ... == state(M_n) == state(X_{ad})$, for
%	any two points in time $v$ and $w$, so that $v+t<w$ there exists a point in time
%	$z$, $v<z<w$ such that $state_z(M_1) == state_z(M_2) == ... == state_z(M_n) ==
%	state_z(X_{ad})$.
%\end{definition}
%
%T-stabilizing shields are hard to achieve in reality, as both the specification
%and the considered fault models need to be synchronizable. However, by only
%considering the core parts of safety-critical systems, one can create small
%automata which satisfy these conditions, and thus ensure that the shield only
%interferes if these most critical parts are violated, and hands back control
%within limited time, in case the violation was according to one of the
%considered fault models.
%

\iffalse
\textbf{before Tina touched it!!!!!!!!!!!!!!!!!!}
In this section, we will show how to generate timed post-shields (as seen in Figure~\ref{fig:attach_shield}(a)), that is, shields that are attached after the system, and monitor and correct all outputs towards the environment. We will introduce three types of shields, \textit{pure safety}, \textit{guaranteed recovery} and \textit{guaranteed time-bounded recovery}, and discuss how these shields can be generated by using the
\textit{refinement} preorder on the specification and a set of considered fault
models. We first define the goals for the three types of shields, then we show how to produce the corresponding strategies, and afterwards we show how these strategies can be converted into timed post-shields.
bla bla bla bla

%\begin{figure}
%	\begin{center}
%		\includegraphics[width=0.45\linewidth]{images/attach_shield.pdf}
%		\caption{Shielding a system.}
%		\label{fig:overview}
%	\end{center}
%\end{figure}

\subsection{Criteria for shields}

The most important criteria that all shields have to abide by is \textit{safety}. A shield provides safety with regards to a given specification, if for any given system, the shield will correct its outputs, so that the corrected outputs, which are the outputs observed by the environment satisfy the specification.

The second criteria that all shields need to conform to is \textit{no unnecessary deviation}, guaranteeing that if no fault was detected, the shield will not correct any of the systems outputs.

Shields with \textit{guaranteed recovery}, in addition to providing safety, come with a guarantee that after a fault the shield will eventually reach the same state as the system again, and thus can hand back control to the original controller. In our case, this can be guaranteed under the assumption, that the system fault was captured by one of out fault models.

Finally, shields with \textit{guaranteed time-bounded recovery}, will in addition guarantee that the state of the system and the shield can be aligned within a given time bound.


\subsection{Pure Safety Strategy}

First we show how to synthesize a pure safety strategy, focused only on shielding incorrect outputs without integrating minimal interference.

We are given a \textbf{system} \sys and a \textbf{specification} \spec. To guard against the unlikely case that \sys does not satisfy, i.e., refine, \spec,
we want to synthesize a \textbf{shield} that will enforce \spec to be satisfied.

In the timed post-shield setting, the shield will receive the output of \sys and forward a (maybe) corrected output to the environment. To differentiate the outputs given by the system and those given by the shield, we will prime outputs given by the shield. To ensure that these primed outputs are safe, we need a variant of the specification \specp that specifies the behavior with respect to these primed outputs. This specification can be transformed
into a monitor \mspecp.

\begin{figure}[tb]
	\begin{center}
		\includegraphics[width=0.5\linewidth]{images/ctr.eps}
		\caption{The control options of the shield.}
		\label{fig:ex_shield}
	\end{center}
\end{figure}

As a next item, we may construct an automaton \shield, depicting the control options for the
shield. This is the only component containing controllable transitions. \shield is produced 
in a manner to enforce no unnecessary deviation, once an error was detected. This is done by guarding its transitions, and only allowing for free choice of the controlled outputs, in case of an error or when an invariant is about to be violated. Otherwise the shield has to follow the outputs given by \sys. 

 

An example of the \shield component for the light switch is depicted in Figure~\ref{fig:ex_shield}.The right two
transitions show the behavior before a fault was detected. In those cases,
\shield will simply forward the outputs it received from the system. If an error
was detected, the two transitions in the top right corner will be enabled, and
\shield can choose any output at any time. The two transitions in the bottom
right show the case where the specification reached a time bound, in which case
\shield is allowed to take over, as a fault of the system might be imminent.

% Finally, we need models of the system and the environment. The model of the environment $\env$ can send input at any time. An example of this can be seen in Figure~\ref{fig:sysenv}(a). If more knowledge of the environment were available, the model could also be more refined by, e.g., only sending a signal at most every second. However, if such an environment was used, a violation of the modelled assumption might lead to safety violations not covered by the shield.

% Next we need a model of \sys. Again, this is the most permissive model, shown in Figure~\ref{fig:sysenv}(b), able to produce any output at any time. This ensures that we will guarantee safety for any outputs we might receive from a system. 


% \begin{figure}
	
	% \minipage{0.49\textwidth}
	% \centering
	% \includegraphics[width=0.7\linewidth]{images/env.eps}\\
	% (a)
	% \endminipage\hfill
	% \minipage{0.49\textwidth}
	% \centering
	% \includegraphics[width=0.7\linewidth]{images/sys.eps}\\
	% (b)
	% \endminipage\hfill
	
	% \caption{A most permissive environment (a) and system (b) for the light controller. }
	% \label{fig:sysenv}
% \end{figure}

We can now consider the timed game given by the following composition:

$$\mathcal{G} = ~\mspec~|~\mspecp~ |~\shield$$

In this game we can observe the shielded system  through the corresponding
monitors. We can both monitor whether the original system satisfies the specification (\spec) and whether the shielded system will satisfy
the primed specification (\specp). We can now find strategies for $\mathcal{G}$
that ensure safety.

For pure \textbf{safety}, the control objective is to ensure that \specp is
never violated by the shielded system. This can be expressed via the following safety 
query specifying that the error state can never be reached. The query is given in the syntax used by \uppaaltiga.
$$
\uppProp{control: A \Box~ \neg \mspecp.\uppLoc{ERR}}
$$

Solving the safety game with respect to this query will produce a strategy $\omega_S$, which will be used in Subsection~\ref{sec:convert} to produce a timed post-shield $Sh_P$ guaranteeing  safety. 






\subsection{Guaranteed Recovery Strategies}

In this section we discuss how to enforce that the shield operates "with minimal
deviation", e.g., while no fault was observed or when a fault is resolved, the
shield should not interfere with the behavior of \sys and a fault should be
resolved as soon as possible. This minimal restriction of \sys is of high
importance, as \sys might be significantly more refined than \spec, and
might, for instance, have been created via machine learning.

To \textit{resolve} an error, we need to know when it is safe to hand back control. In our approach, we achieve this by keeping track of a set of fault models, under the assumption that the error that occurred was captured by one of the fault models. However, since \sys is considered a black-box we cannot observe its internal state. We can thus not know which fault model captured the fault that occurred. Thus, we can only hand back control in case all fault models \textit{align}, that is, they all reached the same state again, and our shielded specification reached the same state as well. To achieve this, the fault models will be updated according to the behavior of \sys and continuously be monitored.

We now can \textit{guarantee} a safe and time-bounded recovery of a (faulty)
\sys, under the following assumptions:
\begin{itemize}
	\item \sys essentially satisfies \spec, except for a single \textit{transient} fault.
	\item The fault that appears in \spec is covered by one of the fault models
	\fspec, with $f \in {f_1,...,f_n}$, we consider. These models are copies of spec with a transient fault connecting the pre-fault behaviour to the post-fault behaviour. 
\end{itemize}

\begin{figure}[tb]
	
	%\minipage{0.89\textwidth}
	\centering
	\includegraphics[width=0.85\linewidth]{images/M1.eps}\\
	%(a)
	%\endminipage\hfill 
%	\\
%	\minipage{0.79\textwidth}
%	\centering
%	\includegraphics[width=0.99\linewidth]{images/mM1.eps}\\
%	(b)
%	\endminipage\hfill
	
	\caption{Transient fault: an unexpected output resets a clock and its monitor. }
	\label{fig:fault}
\end{figure}

An example of a fault model can be seen in Figure~\ref{fig:fault}. The example shows a fault, where an \uppSync{off} signal is produced in the \uppLoc{OFF} location, where it was not allowed. In this example, the faulty signal additionally resets the clock \uppClock{x}, but does not change the location of the automaton, i.e., it still leads to the \uppLoc{OFF} location in the post-fault behavior part of the model.

The fault models can be transformed into monitors \mfspec in the same way the
specification was transformed.% An example is shown in Figure~\ref{fig:fault} (b). 

Now we can consider the timed game given by the following composition:

$$\mathcal{G} = mSpec^{f_1}~|...|~mSpec^{f_n}~|~\mspec~|~\mspecp~ |~\shield$$

In this game we can observe conformance of the system with respect to the fault
models, as well as the original specification (\spec) through the corresponding
monitors. In addition, we can monitor whether the shielded system will satisfy
the specification (\specp). Now we want to find strategies for $\mathcal{G}$
that ensure safety, guaranteed recovery and guaranteed time-bounded recovery.


For \textbf{guaranteed recovery}, we need to establish a state where all
active\footnote{A fault model is active, if its monitor is not in the \uppLoc{ERR}
	location} fault models agree with each other and the \specp, that is, they are all in the same location with the same clocks. This can be achieved with the following leads-to property~\cite{behrmann2004tutorial}, specifying that if we observe a fault, this will eventually lead to recovery. 
\begin{align*}
	&\uppProp{\neg \mspecp.\uppLoc{ERR} \wedge \mspec.\uppLoc{ERR}~leadsto} \\ 
	&\uppProp{(\forall i. [\mspec^{f_i}.\uppLoc{ERR}~ \vee~ (\mspec^{f_i}.\uppVar{l} == \mspecp.\uppVar{l} ~\wedge
	~\mspec^{f_i}.\uppClock{x} = \mspecp.\uppClock{x})])}
\end{align*}

Solving the safety game with respect to this query will produce a strategy $\omega_g$, which will be used in Section~\ref{sec:convert} to produce a timed post-shield $Sh_g$ guaranteeing  safety and eventual recovery. 

Note that if a fault model is inactive, i.e., it reached its error-state, this means that \sys performed an output that was not valid in the fault model. This indicates that the fault model was not a correct prediction of the fault in the system, and can be discarded.


Finally, to achieve \textbf{guaranteed time-bounded recovery} within the bound
\uppVar{T}, we use the following timed leads-to property, specifying that a fault will lead to recovery within $T$ time units:
\begin{align*}
	&\uppProp{\neg \mspecp.\uppLoc{ERR} \wedge \mspec.\uppLoc{ERR} ~leadsto_{\leq T}} \\ 
	&(\forall i . [\mspec^{f_1}.\uppLoc{ERR} ~\vee~ (\mspec^{f_1}.\uppVar{l} == \mspecp.\uppVar{l} ~\wedge
	~\mspec^{f_1}.\uppClock{x} = \mspecp.\uppClock{x})])
\end{align*}

Solving the safety game with respect to this query will produce a strategy $\omega_{gt}$, which will be used in Subsection~\ref{sec:convert} to produce a timed post-shield $Sh_{gt}$ guaranteeing safety and recovery within \uppVar{T} time units. 

%Solving any of these queries on the timed game $\mathcal{G}$ will produce a memoryless strategy $\omega$, collecting a set of permitted actions for each state. A %strategy can be turned into a post-posed or preemtive timed shield $Sh$, which will be discussed in Sections~\ref{sec:postposed} and ~\ref{sec:preempt}, %respectively.

\subsection{Producing a Timed Post-Shield}
\label{sec:convert}

We now will discuss the transformation of a strategy $\omega_{p}$, $\omega_{g}$ or $\omega_{gt}$, into a pure safety shield, a timed shield with guaranteed recovery, and a timed shield with guaranteed time-bounded recovery, respectively.

The need for the three different types of shields arises from two factors. Firstly, guaranteed recovery is not always possible. An obvious example demonstrating this would a system that never resets one of its clocks. If a fault occurred that changes the value of this clock, synchronization can never occur. Secondly, the complexity of creating a shield with guaranteed (time-bounded) recovery is high, and for larger systems / specifications, will not be feasible. However, in such a case usually the pure safety game can still be solved. Thus, the choice of shield depends on the safety-criticality of the system and its complexity.

A shield is derived from the safety game $\mathcal{G}$, which is a network of timed game automata. Since the environment and the system will not be part of the shield, they are removed from the network, leaving us with $\mathcal{G} = \mspec~|~\mspecp~ |~\shield$ in the case of pure safety, and $\mathcal{G} = ~\mspec^{f1}~|...|~\mspec^{fn}~|~\mspec~|~\mspecp~ |~\shield$ in the case of a shield with guaranteed recovery.

\begin{definition}
A shield $Sh$ is the network of timed automata received by composing $\mathcal{G}$ with the derived strategy $\omega$, denoted by $\mathcal{G}\|\omega$, meaning that all unsafe transitions (or transitions that would not lead to recovery) are restricted.
\end{definition}

A shield can be applied after any system, shielding its outputs towards the environment.

Independently on the used type of shield, the following theorem holds for any shield $Sh$ derived this way:

\begin{theorem}
$$(\sys~|~Sh)~ \leq \specp$$
\end{theorem}

That is, for any system \sys, regardless of which fault(s) it contains, if it is placed in parallel with the shield, we will guarantee that it satisfies the specification. 

In addition, we guarantee that we only interfere with the system, in case a fault was detected. We denote by $\textrm{out}$ the timed sequence of outputs received from $\sys$ and by $\textrm{out'}$ the timed sequence of outputs produced by the shield.

\begin{theorem}
$$\neg \mspec.\uppLoc{ERR} \implies \textrm{out} = \textrm{out'} $$
\end{theorem}


Finally, if $Sh$ is a shield with guaranteed (time-bounded) recovery, we have that:
\begin{theorem}
	$$ \exists n : \sys \leq \spec^{fn} \implies (\sys~|~Sh~) \leq \specp \wedge \mspec.\uppLoc{ERR}~\uppProp{leadsto}_{(\leq T)} \textrm{recovery}$$
\end{theorem}

That is, if the system refines any of our considered fault models, in addition to guaranteeing safety, we guarantee that an observed error will lead to recovery (within the time bound \uppVar{T}), where recovery means that all active fault models will be in the same state as the specification. 



\subsection{Fault models}
\input{faultmodels}

% \subsection{Generating shields in UPPAAL Stratego}
% \todo{probably not needed}

% In this section we show how t-stabilizing shields can be produced in UPPAAL Stratego. This will be demonstrated on the example already shown in Figure~\ref{fig:example_kim} and ~\ref{fig:ex_shield}.

% To make the approach work in UPPAAL, we need to produce a monitor that constantly checks whether the system has recovered, by checking whether the conditions for recovery is met and setting an according flag in case. The condition for recovery is that for each fault model either the fault model is inactive, or it is in the same state as the specification. Since guards in UPPAAL do not permit disjunction, the monitor contains several transitions containing the different cases. Only two of these transitions are illustrated in Figure~\ref{todo}.

% The final query used to synthesize a shield with guaranteed time-bounded recovery is given below. It is a rewritten, yet equal, form of the query to the one presented earlier.
% \begin{align*}
% \textrm{strategy REC = }& \textrm{control: } A[]  \textrm{not mSpecp.ERR and} \\ 
% &(( \textrm{not mSpec.ERR})  \textrm{ or } t<=T  \textrm{ or recovered})
% \end{align*}
% This will produce a safety strategy, which can then be exported and used as a shield. The format of the exported strategy is a list of reachable states with a set of attached (sometimes time-guarded) actions that are permitted in the given state, including the option to delay, if it is permitted by the invariants and allowed by the strategy. An extract showing a (slightly simplified) example of the output is shown below:

% \begin{align*}
% \textrm{State:} & ( \textrm{mSpec.ERR mSpecp.ON ... ) error=1 recovered=0 states=1 ...} \\
% & \textrm{When (1 \textless=xs \&\& xs\textless=5), Shield.\_id7-\textgreater Shield.\_id7 \{ error == 1, off\_p!, 1 \}} \\
% &\textrm{mSpecp.ON-\textgreater mSpecp.OFF \{ xs \textgreater= 1, off\_p?, xs := 0, states := 0 \}}\\
% &\textrm{While you are in	(xs\textless 1), wait.}
% \end{align*}


% A complete UPPAAL model containing four fault models and all needed components is available online~\footnote{TODO: upload and add link}. The calculation of a timed shield with guaranteed time-bounded recovery for that example took $9.6$ seconds. This is, admittedly, a very long time for this very small example, and proofs the argument we made earlier, that guaranteed time-bounded recovery is only suitable for the most critical components in larger systems, and cannot be applied to the complete system at once. Comparatively, producing a timed shield with only guaranteed recovery only takes $0.004$ seconds (after pruning the fault models from the UPPAAL model, as they are not used for the pure safety game). 




%
%\section{Demonstrating example}
%\label{sec:demoex}
%
%In this section, we illustrate the challenges associated with shield synthesis
%for timed systems on a simple controller for a light switch.
%Figure~\ref{fig:example_impl}(a) shows the environment, which might randomly
%turn the light on, and receives the on and blink signal from the shield.
%Figure~\ref{fig:example_impl}(b) shows the specification automaton of the light
%switch: whenever the light is switched on,  this setting has to be kept for $1$
%to $5$ time units, and whenever the light is switched off, the light switch has
%to blink at least once every $3$ time units.
%Note, that this is an abstract specification with loose timing constraints. The
%actual \implementation might turn of the light, if the movement in the room has
%ceased.
%
%\begin{figure}
%	
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/spec.eps}
%	% \endminipage\hfill
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/impl}
%	% \endminipage\hfill
%	% \\
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/FM1}
%	% \endminipage\hfill
%	% \minipage{0.49\textwidth}
%	% \centering
%	% \includegraphics[width=0.7\linewidth]{images/FM2}
%	% \endminipage\hfill
%	
%	% \caption{Specification (a) and \implementation (b) and two fault models
%	%(c,d) of the light switch.}
%	\includegraphics[width=0.99\linewidth]{images/shield_ex.png}
%	\caption{Environment (a), Specification (b), two possible faulty
%		implementations(c,d) and four fault models (e,f,g,h) of the light switch.}
%	\label{fig:example_impl}
%\end{figure}
%
%
%Next, lets consider a simple but faulty \implementation of the light switch as
%depicted in Figure~\ref{fig:example_impl}(c), where the red transition in the
%initial state shows the transient error that might appear.
%After two steps, the faulty \implementation outputs an $\textbf{off!}$, without
%an initiating $\textbf{on?}$ signal.
%Since this output would violate the specification, the shield has to interfere
%and to skip the $\textbf{off!}$ signal of the \implementation.
%
%% \begin{figure}
%% \minipage{0.24\textwidth}
%% \includegraphics[width=\linewidth]{images/FM1}
%% \endminipage\hfill
%% \minipage{0.24\textwidth}
%% \includegraphics[width=\linewidth]{images/FM2}
%% \endminipage\hfill
%
%
%% \caption{Two fault models  of the light switch.}
%
%% \label{fig:example_fms}
%% \end{figure}
%
%
%
%The goal of the shield is to produce an output trace, that is not only correct,
%but also leads the shield to a state in which the future signals
%of the \implementation that are correct satisfy the specification again, such
%that the shield can hand back control to the \implementation.
%In order to do that, the shield needs to align with the actual state of the
%\implementation after the fault. The tricky part is that the \implementation is
%considered as a black box and the shield can only observe the output of the
%\implementation.
%In order to determine what that state might be, we launch several fault models,
%assuming that one of them mimics the faulty \implementation. While the shield is
%active, these fault models are simulated according to the inputs and the outputs
%of the \implementation.
%If a fault model can not follow the output of the \implementation (including not
%allowing a delay that is possible in the \implementation), it was not the
%correct fault model for the observed fault and is discarded.
%Only if all non-discarded fault models agree on the same state and the shield
%has reached that state as well, can we tell that the shield and the
%\implementation have synchronized again.
%
%We give four possible fault models in Figure~\ref{fig:example_impl}(e,f,g,h).
%The first fault model assumes that the output happened and reset the clock, but
%that the \implementation still is in location $\textbf{OFF}$. The second one
%assumes that the fault led the \implementation to location $\textbf{ON}$,
%reseting the clock. The next two fault models are the same, but without reseting
%the clock. 
%
%The slightly adapted specification and the fault models form a network of timed
%game automata. The shield is computed by playing a timed game on this network,
%with the goal of reaching the state of the fault models as fast as possible. The
%outputs of the shield, which are provided to the environment, are marked via an
%overline.
%
%Table~\ref{tbl:example} shows a possible execution of the shielded faulty light
%switch.
%After 2 time units a wrong output is produced, the shield corrects the output
%and all automata, except the second and fourth fault model, enter location
%$\textbf{OFF}$ but with differing clock values. The shield corrects the output
%and immediately gives  a $\textbf{$\overline{blink}$!}$ output instead, which
%only changes the state of the shield itself.
%After $1$ time unit, the environment gives the input $\textbf{on?}$ and all
%automata enter the same location, but fault models $2$ and $4$ have a different
%clock value.
%The shield is still in control, but unless the \implementation gives an
%$\textbf{off!}$ signal, the most beneficial option for the shield is to wait for
%that signal, in order to follow it.
%After two seconds of waiting, the invariant of fault model $4$ is broken, and
%the fault model can be discarded.
%As soon as the \implementation sends the $\textbf{off!}$ signal, all remaining
%fault models are in the same state and the shield can follow them by creating
%the $\textbf{$\overline{off}$!}$ output. Now all automata are aligned and we can
%hand back control to the actual \implementation.
%
%\begin{table}
%	\centering
%	\begin{tabular}{ | c | c | c | c | c | c |  c | }
%		\hline
%		timed trace  & init & (2,off!) & (0,$\overline{blink}$!)  & (1,on?)    & (3,
%		off!) & (0, $\overline{off}$!) \\ \hline % (5,off!) | (5,off'!)
%		Impl.1  & (OFF, x=0) & (OFF, x=0) & (OFF, x=0)            & (ON, x=0)  & (OFF,
%		x=0)  & (OFF, x=0) \\ % & (l0, x=0) \\
%		Shield  & (OFF, x=0) & (OFF, x=2) & (OFF, x=0)            & (ON, x=0)  & (ON,
%		x=3)   & (OFF, x=0) \\ % & (l0, x=0)  \\
%		FM1  & -             & (OFF, x=0) & (OFF, x=0)            & (ON, x=0)  & (OFF,
%		x=0)  & (OFF, x=0)  \\ %& x  \\
%		FM2  & -             & (ON, x=0)  & (ON, x=0)             & (ON, x=1)  & (OFF,
%		x=0)  & (OFF, x=0) \\% & (l0, x=0)  \\
%		FM3 & - 			  & (OFF, x=2) & (OFF, x=2)            & (ON, x=0)  & (OFF, x=0)  &
%		(OFF, x=0)\\
%		FM4 & -              & (ON, x=2)  & (ON, x=2)             & (ON, x=3)  &
%		\frownie{}  & \frownie{}\\% & (l0, x=0)  \\
%		
%		\hline
%	\end{tabular}
%	\caption{A possible shielded execution of the light switch with the faulty
%		\implementation $1$.}
%	\label{tbl:example}
%\end{table}
%
%Table~\ref{tbl:example2} shows a possible execution, where we assume the
%\implementation behaved like faulty \implementation $2$. The fault models are
%again initialized after a two second delay followed by the faulty
%$\textbf{off!}$ signal. Assuming that we do not receive an $\textbf{on?}$
%signal, the shield could simply loop with $\textbf{blink!}$ signals, and wait
%for all other models to collect in the $\textbf{OFF}$ location, thus, let us
%assume after one second an $\textbf{on?}$ signal arrives. While all automata are
%in the same location, there is a one second delay between the shield and the
%\implementation. This means that the \implementation can leave the location with
%an $\textbf{off!}$ signal one second earlier than the shield can follow. As soon
%as the shield follows it with an $\textbf{$\overline{off}$!}$ signal, the
%\implementation can already move back to the \textbf{ON}$ state, and the shield
%will never be able to catch up. Thus, in this case no t-stabilizing shield can
%exist, and unless the environment helps us at some point by delaying the
%\textbf{on?}$ signal long enough for the shield to wait the \implementation in
%the $OFF$ location, we will not be able to give back control.
%
%\begin{table}
%	\centering
%	\begin{tabular}{ | c | c | c | c | c | c |  c  | }
%		\hline
%		timed trace  & init & (2,off!)     & (1,on?)    & (1, off!) & (1,
%		$\overline{off}$!) & ... \\ \hline % (5,off!) | (5,off'!)
%		Impl.2  & (OFF, x=0) & (ON, x=0)   & (ON, x=1)  & (OFF, x=0)  & (OFF, x=1) &
%		... \\ % & (l0, x=0) \\
%		Shield  & (OFF, x=0) & (OFF, x=2)  & (ON, x=0)  & (ON, x=1)   & (OFF, x=0) &
%		... \\ % & (l0, x=0)  \\
%		FM1  & -             & (OFF, x=0)  & (ON, x=0)  & \frownie{}  & \frownie{} &
%		...  \\ %& x  \\
%		FM2  & -             & (ON, x=0)   & (ON, x=1)  & (OFF, x=0)  & (OFF, x=1) &
%		... \\% & (l0, x=0)  \\
%		FM3 & - 			  & (OFF, x=2)  & (ON, x=0)  & \frownie{}  & \frownie{} & ...\\
%		FM4 & -              & (ON, x=2)   & (ON, x=3)  & (OFF, x=0)  & (OFF, x=1) &
%		...\\% & (l0, x=0)  \\
%		
%		\hline
%	\end{tabular}
%	\caption{A possible shielded execution of the light switch with the faulty
%		\implementation $2$.}
%	\label{tbl:example2}
%\end{table}
%
%
%\section{Timed Shields}
%
%In this section we will propose algorithms for the generation of three types of
%shields, a general shield that only cares about satisfying the specification,
%and two more advanced shields that rely on fault models in order to determine
%when / if they can give back control to the shielded controller. For that we
%assume a set of fault models $M_n$, and a safety specification $Spec$. 
%
%\subsection{General Timed Shields}
%
%General timed shields are a basic form of runtime enforcement, as they do not
%take over control for a given time, but simply overwrite any outputs that do not
%satisfy the specification. This means, they symbolize the most permissive
%strategy~\ref{test} of the system, that satisfies the specification.
%
%\begin{definition}[General timed shields]
%	A general timed shield $X_g$, is the most permissive refinement of $Spec$, i.e.,
%	$X_g \leq_{mp} Spec$.
%\end{definition}
%
%The advantage of general timed shields is that they need less information about
%the actual implementation or possible faults. This makes them very usable for
%the shielding of controllers that were derived via machine learning. 
%
%\subsection{Admissible Timed Shields}
%
%Admissible timed shields use the fault models in order to determine when control
%can be given back to the controller. They will shield the system until all
%(non-discarded) fault models are in the same state as the shield. However, there
%is no guarantee for this to ever happen, and some cooperation from the
%environment might be necessary to achieve it.
%
%\begin{definition}[Admissible timed shields]
%	An admissible timed shield is the component $X_{ad}$, so that $(M_1 || M_2 ||
%	... || M_n || X_{ad}) \leq_{mp} Spec$ and \textbf{$\overline{o}$!}$ ==
%	\textbf{o!}$ whenever $state(M_1) == state(M_2) == ... == state(M_n) ==
%	state(X_{ad})$.
%\end{definition}
%
%Admissible shields are to be used, when the considered fault models are not
%synchronizing timed automata. In most practical cases, the environment will not
%actively try to keep the automata from synchronizing, thus, the shield will most
%likely have a chance of aligning its state with the implementation eventually. 
%
%\subsection{T-stabilizing Timed Shields}
%
%T-stabilizing timed shields guarantee to give back control within t-timesteps.
%They will shield the system until all (non-discarded) fault models are in the
%same state as the shield, but never longer than for $t$ time units in a row. 
%
%\begin{definition}[T-stabilizing timed shields]
%	A t-stabilizing timed shield is the component $X_{ts}$, so that $(M_1 || M_2 ||
%	... || M_n || X_{ts}) \leq_{mp} Spec$, \textbf{$\overline{o}$!}$ == \textbf{o!}$
%	whenever $state(M_1) == state(M_2) == ... == state(M_n) == state(X_{ad})$, for
%	any two points in time $v$ and $w$, so that $v+t<w$ there exists a point in time
%	$z$, $v<z<w$ such that $state_z(M_1) == state_z(M_2) == ... == state_z(M_n) ==
%	state_z(X_{ad})$.
%\end{definition}
%
%T-stabilizing shields are hard to achieve in reality, as both the specification
%and the considered fault models need to be synchronizable. However, by only
%considering the core parts of safety-critical systems, one can create small
%automata which satisfy these conditions, and thus ensure that the shield only
%interferes if these most critical parts are violated, and hands back control
%within limited time, in case the violation was according to one of the
%considered fault models.
%
\fi

==> faultmodels.tex <==


Since the shield only monitors the output of the implementation, after an error it has no information on what the system intended to do
and what state the system currently is in. It could be that e.g., (1) the output was wrong because of a transmission error and the
system  traversed according to one of the valid transitions, but the shield does not know which one, or (2) the output was a fluke and the
system did not change its state at all, or (3) that a deadline was missed by a delayed output, or (4) that a timer was erroneously reset.  
However, in order to be able to guide the current execution back to a state where the shield can end deviation and hand back control to the implementation,
the shields need ways of determining the current state of the implementation.
This idea is based on the assumption, that after the error the system behaves correctly again. Thus, if the shield and the system reach  the same state, it would be desirable for the system to take over.

In order to figure out the current state of the system, the erroneous transition leads to a different state in each fault model. Each one monitors one possible state the system could possibly be in after the fault. 
The fault models continue to monitor the behavior of the system during execution. 
As soon as a fault model can not follow the output of the implementation, it was not the correct fault model for the observed fault and
is discarded. 
Only if all active fault models agree on the state, we have presumably found the state the system is currently in.

\iffalse

In this paper, we focus on the location faults: go-to-any-location faults and go-to-next-location faults; and on the
clock faults:  wrong-reset faults and binary-swapped-clocks faults. We leave the discussion of the other fault models and their combination to future work. 

Each of the faults we consider induces a set of possible states the implementation could be in. We define the function
$\textrm{FM}(\A_\varphi):\locs{}_\varphi\times\posreals^{\clocks_\varphi}\rightarrow2^{\locs{}_\varphi\times\posreals^{\clocks_\varphi}}$ that computes the set of states to be monitored, for each type of fault we consider.

$\textrm{FM}(\A_\varphi, \loc_\varphi, \val_\varphi) :=$ \\
\begin{align}
 \{(\loc, \val_\varphi)\mid  & \loc\in\locs{}_\varphi \wedge \loc \neq \loc_\varphi \} \text{ for \emph{Go-to-any-location} faults.}\\
  \{(\loc, \val)\mid  & \loc\in\locs{}_\varphi \wedge \exists (\loc_\varphi, \val_\varphi) \xrightarrow{\oaction{a}}(\loc, \val)  \} \text{ for \emph{Go-to-next-location} faults.}\\
 \{(\loc_\varphi, \val)\mid & \exists x_i : \val(x_i)=0 \wedge \forall x_{j \neq i} : \val(x_j) = \val_\varphi(x_j) \}  \text{ for \emph{Wrong-reset} faults.}\\
\{(\loc_\varphi, \val)\mid  & \exists x_i,x_j : \val(x_i)=\val_\varphi(x_j), \val(x_j)=\val_\varphi(x_i) \wedge \\
& \forall x_{k \neq i,j}: \val(x_k) = \val_\varphi(x_k) \}   \text{ for \emph{Binary-swapped-clocks} faults.}
\end{align}
All of these fault types can be combined arbitrarily.
However, the more fault types that are used, the higher the complexity will be for the shield synthesis problem, as the set of states to be monitored grows larger.

For $(\loc_\varphi, \val_\varphi)$, we introduce a fault model for each state  $(l,v)\in\mutants(\A_\varphi, \loc_\varphi, \val_\varphi)$.
Each fault model corresponds to a copy of the specification automaton $\A_\varphi$, but uses $(l,v)$ as its initial state.



$\mutants(\A_\varphi, \loc_\varphi, \val_\varphi) =$ \\
\begin{align}
 \{(\loc, \val_\varphi)\mid  & \loc\in\locs{}_\varphi \wedge \loc \neq \loc_\varphi \} \cup\label{fault:gotoany}\\
  \{(\loc, \val)\mid  & \loc\in\locs{}_\varphi \wedge \exists (\loc_\varphi, \val_\varphi) \xrightarrow{\oaction{a}}(\loc, \val)  \} \cup\label{fault:gotonext}\\
 \{(\loc_\varphi, \val)\mid & \exists x_i : \val(x_i)=0 \wedge \forall x_{j \neq i} : \val(x_j) = \val_\varphi(x_j) \} \cup\label{fault:wrongresets}\\
\{(\loc_\varphi, \val)\mid  & \exists x_i,x_j : \val(x_i)=\val_\varphi(x_j), \val(x_j)=\val_\varphi(x_i) \wedge  \\
& \forall x_{k \neq i,j}: \val(x_k) = \val_\varphi(x_k) \} \label{fault:binaryswap}
\end{align}

 Line~\ref{fault:wrongresets} all {\em wrong reset} faults and Line~\ref{fault:binaryswap} all {\em binary swapped clocks} faults. For the illustrative example provided in Section~\ref{sec:demoex}, the corresponding numbers of fault models while in location $\textbf{l0}$ would be $2$, $1$, $1$ and $0$, respectively.
\fi


==> images/coordinator.tex <==
\begin{tikzpicture}[
every node/.style = {
		     shape=rectangle,% is not necessary, default node's shape is rectangle
                     draw=gray, very thick,
                     inner sep=.2cm,
                     rounded corners=3mm,
                     align=center,
                     font=\sffamily
}]

\node (unshielded) at (0,0) {\begin{tabular}{c}
Unshielded\\
$\N=\A_S$
\end{tabular}};

\node (shielded) at (6,0) {\begin{tabular}{c}
Shielded\\
$\N'=\A_S\|\A_F^0\|\dots \A_F^n$
\end{tabular}};

\path[->,thick,black] (-2,0) edge (unshielded);

\path[->,thick,black,bend left=30] (shielded) edge node[draw=none, below, yshift=0pt] {
\begin{tabular}{c}
Immediately when Equation~\ref{eq:allok} is true\\
Emit $\allok!$\\
let $q'=(s_S,s_1,\dots,s_n)$ be the state of the NTA $\N'$\\
$\N=\A_S$ with state $q=(s'_S)$ where $s_S\trans{\allok}s'_S$.
\end{tabular}
} (unshielded);

\path[->,thick,black,bend left=30] (unshielded) edge node[draw=none, above, yshift=0pt] {
\begin{tabular}{c}
Received $\startfm?$\\
let $q=(s_S)$ be the state of the NTA $\N$\\
let $\{s_0,\dots, s_n\}=\mutants(s_S)$\\
$\N'=\A_S\|\A_F^0\|\dots \A_F^n$ with $q'=(s_S,s_0,\dots,s_n)$.
\end{tabular}
} (shielded);

\end{tikzpicture}

==> images/shielded.tex <==
\begin{tikzpicture}[
every node/.style = {
		     shape=circle,% is not necessary, default node's shape is rectangle
                     draw=black, thin,
                     align=center,
                     minimum size=3mm
},xscale=0.7]



\begin{scope}[shift={(0,0)}]
\node (ol) at (0,0) {$\ell$};
\node (olo1) at (0,-3) {$\ell_{\alpha}$};
\node (old1) at (0,-6) {$\ell'$};
\node (ole) at (6,0) {$\ell_\tau$};


\path[->,thick,black,dashed] (ol) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\true,\alpha?,\emptyset)$} (olo1);
\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\psi,\overline{\alpha}!,X)$} (old1);

\path[->,thick,black] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-1cm] {$(\lastbound(\invars{}_\varphi(\ell)),\tau!,\emptyset)$}  (ole);

\end{scope}

\node[draw=none,font=\fontsize{30}{0}\selectfont] at (5.5,-3) {$\implies$};

\begin{scope}[shift={(10,0)}]
\node (ol) at (0,0) {$\ell$};
\node (olo1) at (0,-3) {$\ell_{\alpha}$};
\node (old1) at (0,-6) {$\ell'$};
\node (ole) at (7,0) {$\ell_\tau$};

\node (sl) at (7,-3) {$\overline{\loc}$};
\node (sle) at (7,-6) {$\overline{\loc'}$};

\path[->,thick,black,dashed] (ol) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\true,\alpha?,\emptyset)$} (olo1);
\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,below,yshift=0.6cm] {$(\psi,\overline{\alpha}!,X)$} (old1);

\path[->,thick,black] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-1cm] {$(\lastbound(\invars{}_\varphi(\ell)),\tau!,\emptyset)$}  (ole);

\path[->,thick,black] (sl) edge node[draw=none,sloped,pos=0.5,below,yshift=0.5cm]  {$(\psi,\overline{\alpha}!,X)$}  (sle);

\path[->,thick,black] (ole) edge node[draw=none,sloped,pos=0.5,below,yshift=.5cm]  {$(\true,\startfm!,\emptyset)$}  (sl);

\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,below,yshift=.4cm]  {$(\overline{\psi},\startfm!,\emptyset)$}  (sl);

\path[->,thick,black] (sl) edge node[draw=none,sloped,pos=0.5,below,yshift=.4cm]  {$(\true,\allok?,\emptyset)$} (ol);

\end{scope}
\end{tikzpicture}

==> images/violation.tex <==
\begin{tikzpicture}[
every node/.style = {
		     shape=circle,% is not necessary, default node's shape is rectangle
                     draw=black, thin,
                     align=center,
                     minimum size=3mm
},xscale=0.7]


\begin{scope}[shift={(0,0)}]
\node (ol) at (0,0) {$\ell$};

\node (oli1) at (-3,-6) {$\ell^1$};
\node[draw=none] at (-2,-6) {\dots};
\node (oli2) at (-1,-6) {$\ell^k$};
\node (olo1) at (1,-6) {$\ell^m$};
\node[draw=none] at (2,-6) {\dots};
\node (olo2) at (3,-6) {$\ell^n$};


\path[->,thick,black,bend right=30] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_1,\alpha_1?,X_1)$} (oli1);
\path[->,thick,black,bend right=10] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_k,\alpha_k?,X_k)$}  (oli2);
\path[->,thick,black,bend left=10] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_m,\alpha_m!,X_m)$} (olo1);
\path[->,thick,black,bend left=30] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_n,\alpha_n!,X_n)$}  (olo2);
\end{scope}

\node[draw=none,font=\fontsize{30}{0}\selectfont] at (5.5,-3) {$\implies$};

\begin{scope}[shift={(12,0)}]
\node (ol) at (0,0) {$\ell$};

\node (oli1) at (-4,-6) {$\ell^1$};
\node[draw=none] at (-3,-6) {\dots};
\node (oli2) at (-2,-6) {$\ell^k$};
\node (olo1) at (2,-3) {$\ell_{\alpha_m}$};
\node[draw=none] at (3,-3) {\dots};
\node (olo2) at (4,-3) {$\ell_{\alpha_n}$};

\node (old1) at (2,-6) {$\ell^m$};
\node[draw=none] at (3,-6) {\dots};
\node (old2) at (4,-6) {$\ell^n$};

\node (ole) at (0,-5) {$\ell_\tau$};

\path[->,thick,black,bend right=40,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_1,\alpha_1?,X_1)$} (oli1);
\path[->,thick,black,bend right=10,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_k,\alpha_k?,X_k)$}  (oli2);
\path[->,thick,black,bend left=10,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\true,\alpha_m?,\emptyset)$} (olo1);
\path[->,thick,black,bend left=40,dashed] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\true,\alpha_n?,\emptyset)$}  (olo2);
\path[->,thick,black] (olo1) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_m,\overline{\alpha_m}!,X_m)$} (old1);
\path[->,thick,black] (olo2) edge node[draw=none,sloped,pos=0.5,above,yshift=-0.7cm] {$(\psi_n,\overline{\alpha_n}!,X_n)$}  (old2);

\path[->,thick,black] (ol) edge node[draw=none,sloped,pos=0.5,above,yshift=-1cm] {$(\lastbound(\invars{}_\varphi(\ell)),\tau!,\emptyset)$}  (ole);

\end{scope}
\end{tikzpicture}

==> postposed.tex <==
In  this section we will show how a safety strategy $\omega$ derived by either of the queries introduced in Section~\ref{sec:ts} can be used as a post-posed timed shield. In post-posed shielding, the shield is applied between the system under shielding and the environment (see Figure~\ref{fig:attach_shield} (a)). Every input and output of the system has to be provided to the shield, in order for the shield to check whether the outputs are safe and overwrite them in case they are not.
In the case of timed shields, additionally all timing constraints need to be observed, and in case an output is to be produced before a given deadline (marked by in invariant in the case of timed automata), the shield may interfere and produce that output at the last moment in time where it is expected, to ensure safety.


In order to use the  produced safety strategy $\omega$ as a shield, we simply need to compose it with the safety game $\mathcal{G}$. The composition $\mathcal{G}\|\omega$ will be a network of timed game automata where all unsafe transitions are pruned. 

Per construction of the component $\sh$, the outputs of the network will always conform to the outputs of the system, unless an error was detected or a timing constraint is about to be violated. Thus, an adapter that uses the network as a shield simply needs to simulate the network during execution of the system, and pass the outputs of the network on to the environment. 



%
% To use UPPAAL Stratego for the shielding, an adapter needs to be developed, that simulates all timed automata in $\mathcal{G}$ in parallel to the system under shielding and uses the strategy to suggest corrected outputs if needed. The intuition behind the adapter is given in Algorithm~\ref{alg:postposed}.
%
%
%\begin{algorithm}[H]
%	\SetAlgoLined
%	
%	\KwIn{Channels $in$, $out$, $out'$, Strategy $\omega$}
%	
%	\While{While true}{
%		\If{condition}{
%			instructions1\;
%			instructions2\;
%		}{
%			instructions3\;
%		}
%	}
%	\caption{How to write algorithms}
%	\label{alg:postposed}
%\end{algorithm}







$\alpha'\in\omega(\loc,\val)$
